A Hierarchical Transformation-Discriminating Generative Model for Few Shot Anomaly Detection

Anomaly detection, the task of identifying unusual samples in data, often relies on a large set of training samples. In this work, we consider the setting of few-shot anomaly detection in images, where only a few images are given at training. We devise a hierarchical generative model that captures the multi-scale patch distribution of each training image. We further enhance the representation of our model by using image transformations and optimize scale-specific patch-discriminators to distinguish between real and fake patches of the image, as well as between different transformations applied to those patches. The anomaly score is obtained by aggregating the patch-based votes of the correct transformation across scales and image regions. We demonstrate the superiority of our method on both the one-shot and few-shot settings, on the datasets of Paris, CIFAR10, MNIST and FashionMNIST as well as in the setting of defect detection on MVTec. In all cases, our method outperforms the recent baseline methods.

==> old.tex <==


%We now consider the importance of the different components of our anomaly scoring function. For this, we consider several variants of our model: (i) 
%In Eq.~\ref{eq:score_3}, given a map of scores $d^n_i(x_{test})$, for each $i$, we first average this map over all pixels (corresponding to image patches). This result in a single score for each $i$ from which we take the maximum score. The final score is the sum of this score over all scales. 
%(ii)  $agg$ operator that returns the 70th percentile of the similarity values,  instead of the 40th percentile.  (iii) To evaluate the contribution of using all the discriminators from the different scales, we consider a variant in which we ignore the discriminator corresponding to scale 0 (the coarsest scale) and another variant, (iv), in which we ignore scale $N$ (the finest scale). The result are reported in Tab.~\ref{tab:ablation}.

% \begin{table*}
% \centering
%  \renewcommand\theadfont{}
% \scalebox{0.8}{%

% \begin{tabular}{ccccccccc}
% \toprule
% Class & \thead{without\\ transformations}   & \thead{without \\ generator}   &  \thead{without \\ generator \& \\ transformations} & CVPR  &  \thead{with GEOM \\ transformations }  & \thead{without \\ hierarchy \\ (min=max=20)} &  \thead{without \\ hierarchy \\ (min=max=100)} & \thead{different \\score?}\\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\
% \toprule\\
% \multicolumn{7}{c} {CIFAR-10 } \\
% \midrule
% Plane & 65.2 $\pm$ 10.6 &  58.9 $\pm$ 12.5 &  &65.2 $\pm$ 5.6 & 63.8 $\pm$ 1.9 &   60.1 $\pm$ 5.9 & 59.9 $\pm$ 9.9 &  \\
% Car   & 65.5 $\pm$ 3.5  &  61.6 $\pm$ 7.8  & & 58.3 $\pm$ 3.6 & 66.2 $\pm$ 4.9 & 63.6 $\pm$ 5.8 & 55.0 $\pm$ 8.6 & \\
% Bird & 56.0 $\pm$ 4.2 &  52.6 $\pm$ 6.3  & & 54.2 $\pm$ 3.2 &  51.9 $\pm$ 4.4 &  48.9 $\pm$ 6.8 & 52.9 $\pm$ 5.9 &\\
% Cat  & 55.7 $\pm$ 3.2  &  53.8 $\pm$ 8.0  & & 56.8 $\pm$ 3.6 & 58.4 $\pm$ 5.8  & 54.3 $\pm$ 5.4& 48.2 $\pm$ 6.6 &\\
% Deer & 55.7 $\pm$ 8.9 &   61.9 $\pm$ 6.8 & & 56.5 $\pm$  10.1 & 53.1 $\pm$ 6.4 & 53.6 $\pm$ 8.1 &67.8 $\pm$ 2.6& \\
% Dog   & 53.0 $\pm$ 4.1 &  61.0 $\pm$ 7.8 &  & 60.0 $\pm$ 3.4 &  61.2 $\pm$ 6.6 & 57.5 $\pm$ 7.6& 55.8 $\pm$ 7.8 &\\
% Frog  & 56.4 $\pm$ 8.1 &  65.1 $\pm$ 9.9  &  & 62.5 $\pm$ 4.2 & 53.8 $\pm$ 5.5& 57.5 $\pm$ 8.1& 62.3 $\pm$ 9.6 & \\
% Horse &53.7 $\pm$ 4.1  &  61.8 $\pm$ 7.8 & & 59.4 $\pm$ 3.5 &  63.2 $\pm$ 6.7& 59.7 $\pm$ 7.8 & 54.6 $\pm$ 7.6&\\
% Ship  & 65.1 $\pm$ 10.2 &  70.4 $\pm$ 9.5  & & 62.6 $\pm$ 7.5 &  71.4 $\pm$ 6.9&  58.1 $\pm$ 8.5 & 69.5 $\pm$ 9.4& \\
% Truck  &    64.8 $\pm$ 4.1  & 60.3 $\pm$ 8.8  & & 61.2 $\pm$ 7.2  &  66.1 $\pm$ 5.5&  59.1 $\pm$ 4.8 & 50.0 $\pm$ 6.2&\\
% \midrule
% Avg   &  59.1  &  60.7 & &  59.7   &    60.9 &  57.3 & 57.6 &\\
% \bottomrule \\
% \end{tabular}}
% \caption{ablation study for \textbf{one} shot - we assess the individual effects of each component of our model (1) the generator (2) applying transformations and training the discriminator to predict them (3) applying  augmentations to training data (4) different kind of anomaly score }
% \label{tab:ablation}
% \end{table*}

% \begin{table*}
% \centering
%  \renewcommand\theadfont{}
% \scalebox{0.8}{%

% \begin{tabular}{ccccccccc}
% \toprule
% Class & \thead{without\\ transformations}   & \thead{without \\ generator}   &  \thead{without \\ generator \& \\ transformations} & CVPR  &  \thead{with GEOM \\ transformations }  & \thead{without \\ hierarchy \\ (min=max=20)} &  \thead{without \\ hierarchy \\ (min=max=100)} & \thead{different \\score?}\\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\
% \toprule\\
% \multicolumn{7}{c} {CIFAR-10 } \\
% \midrule
% Plane & &   &  &  61.4 $\pm$ 3.9 & &    & &  \\
% Car   & &   &  & 70.2 $\pm$ 2.7  & &    & &  \\
% Bird & &  &  & 56.2 $\pm$ 2.4   & &    & &  \\
% Cat & & &  &    58.2 $\pm$ 4.2  & &    & &  \\
% Deer & &  &  &  61.3 $\pm$ 4.9   & &    & &   \\
% Dog   & &   &  &  61.2 $\pm$ 3.9  & &    & &  \\
% Frog & &   &  & 66.3 $\pm$ 6.8 & &    & &  \\
% Horse & &   &  & 63.3 $\pm$ 2.6 & &    & &  \\
% Ship  & &   &  & 67.5 $\pm$ 6.0 & &    & &  \\
% Truck & &   &  & 66.5 $\pm$ 3.7  & &    & & \\
% \midrule
% Avg   &    &   & & 63.4  $\pm$ 4.2  &   &  &  &\\
% \bottomrule \\
% \end{tabular}}
% \caption{ablation study for \textbf{five} shot - we assess the individual effects of each component of our model (1) the generator (2) applying transformations and training the discriminator to predict them (3) applying  augmentations to training data (4) different kind of anomaly score }
% \label{tab:ablation_5shot}
% \end{table*}

% \paragraph{Importance of different components of our model} \shelly{We asses the individual effects of each component the consists of our model: The generator, transformations, multi-scale pyramid. The result are reported in Tab.~\ref{tab:ablation} \\
% \underline{The generator} \quad We consider a variant of our model where we don't use the generator $G$ in our training, only $D$ classifying. The discriminator learns to distinguish between the normal and anomalous images only using the real images. \\

% \noindent \underline{The hierarchy} \quad  we consider a variant of our model where the generation and discrimination is based only on one scale. In out setting, the size of the image size is 128, the min size = 25 and the max size = 64. Since our generative model is based on patches, we consider the two following variants (1) We train our patch based GAN with min size = max size = 20 (16\% of the image size) (2) \textcolor{red}{We train our patch based GAN with min size = max size = 64 (50\% of the image size) } (3) We train our patch based GAN with min size = max size = 100 (80\% of the image size).\\

% \noindent \underline{Transformations} \quad training the model without transformations. just generator, discriminator and multi scale.

% \noindent \underline{CVPR (need to rephrase it)} \quad  instead of transformations as El Yaniv we apply augmentations with probability $p$ during training, and the training loss is WGAN.


% \begin{table*}
% \centering
% \scalebox{0.8}{%
% \begin{tabular}{cccccccc:c}
% \toprule 
% \multicolumn{8}{c:} {MVTec } \\
% \midrule
% Class  & DifferNet & DROCC & Patch-SVDD & Deep-SVDD & GEOM & GOAD & \thead{\textbf{OURS} \\ (score DD)} & \thead{\textbf{OURS} \\ (score DD \\ DifferNet transforms)} \\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\

% \midrule
% Bottle & \textbf{98.2 $\pm$ 0.4} & 67.2 $\pm$ 6.6 & 60.9 $\pm$ 12.3 & 16.6 $\pm$ 5.3& 79.0 $\pm$ 3.5 & 51.6 $\pm$ 14.0 & 76.3 $\pm$ 6.9 & 76.5 $\pm$ 9.0 \\
% Cable & \textbf{76.6 $\pm$ 5.9} & 68.1 $\pm$ 4.3& 58.8 $\pm$ 4.5 & 39.0 $\pm$ 3.5 & 64.2 $\pm$ 1.3 & 47.9 $\pm$ 2.4& 72.3 $\pm$ 3.7 &  67.8 $\pm$ 3.6\\
% Capsule &57.7 $\pm$ 4.6& 50.2 $\pm$ 6.4& 57.9 $\pm$ 12.1& 44.8 $\pm$ 4.4& 55.4 $\pm$ 2.6 &51.2 $\pm$ 3.7 &56.0 $\pm$ 8.4 & \textbf{59.7 $\pm$ 6.2} \\
% Carpet &61.5 $\pm$3.0 &71.9 $\pm$ 10.6&45.5 $\pm$ 18.8 & 41.2$\pm$ 18.2 & 55.0 $\pm$ 10.1 &48.1 $\pm$ 1.9 & \textbf{72.7 $\pm$ 6.7} &  \textbf{81.6 $\pm$ 9.2} \\
% Grid &59.2 $\pm$ 5.1 & 50.0 $\pm$ 4.6&37.2 $\pm$ 12.2 & 79.7 $\pm$ 8.6& 40.1 $\pm$ 13.1 & 9.4 $\pm$ 6.8&73.2 $\pm$ 9.8 & \textbf{83.3 $\pm$ 7.1} \\
% Hazelnut & \textbf{90.7 $\pm$ 2.7} & 66.4 $\pm$ 7.6 & 46.7 $\pm$ 16.1& 29.1 $\pm$ 4.3& 47.8 $\pm$ 3.6 & 47.6 $\pm$ 3.2 & 82.4 $\pm$ 8.7 & 69.3 $\pm$ 10.0 \\
% Leather & 83.4 $\pm$ 1.9& 79.1 $\pm$ 6.5& 61.9 $\pm$ 15.6& 48.0 $\pm$ 3.2&  33.2 $\pm$ 0.5 & 58.1 $\pm$ 6.8& \textbf{98.2 $\pm$ 0.9} & 96.7 $\pm$ 1.8 \\
% Metalnut & 44.4 $\pm$ 8.0& 51.9 $\pm$ 3.6 & 50.4 $\pm$ 13.1 &42.6 $\pm$ 14.7 & 52.3 $\pm$ 4.2 &7.2 $\pm$ 6.5 & \textbf{66.0 $\pm$ 11.0}  & 65.8 $\pm$ 9.9 \\
% Pill & 71.7 $\pm$ 4.4  & \textbf{72.5 $\pm$ 4.0} & 57.6 $\pm$ 8.1& 33.5 $\pm$ 4.0& 67.0 $\pm$ 2.3 & 62.5 $\pm$ 8.1& 56.5 $\pm$ 9.6 &  66.1 $\pm$ 6.9 \\
% Screw & 61.8 $\pm$ 7.7 & 57.7 $\pm$ 9.0 & 53.7 $\pm$ 18.2& 70.1 $\pm$ 10.8& 34.7 $\pm$ 11.1 & 6.3 $\pm$10.0& \textbf{93.5 $\pm$ 6.2} &  89.1 $\pm$ 8.9\\
% Tile & \textbf{87.3 $\pm$ 2.6} & 65.6 $\pm$ 2.0 & 57.3 $\pm$ 4.7 &40.7 $\pm$ 2.8 & 61.0 $\pm$ 2.8 & 6.0 $\pm$ 5.4 & 80.2 $\pm$ 8.2 &  83.0 $\pm$ 8.9 \\
% Toothbrush &52.1 $\pm$ 2.3 & 68.9 $\pm$ 4.5& 63.7 $\pm$ 6.1 & 35.5 $\pm$ 1.5& 65.7 $\pm$ 6.5 & 54.4$\pm$5.4 &67.3 $\pm$ 4.7& 57.5 $\pm$ 5.9 \\
% Transistor & 47.0 $\pm$ 6.5& 59.9 $\pm$ 3.3& 66.7 $\pm$ 14.5 &32.8 $\pm$ 4.3 & 58.1 $\pm$ 1.5 & 61.7 $\pm$ 4.4& 66.1 $\pm$ 7.7 & 67.8 $\pm$ 5.8 \\
% Wood & \textbf{96.0 $\pm$ 2.2} & 70.6 $\pm$ 14.4 & 55.7 $\pm$ 18.4 & 44.0 $\pm$ 16.4& 52.3 $\pm$ 1.1 & 41.8 $\pm$ 6.5& 89.0 $\pm$ 4.2 & 81.7 $\pm$ 9.9 \\
% Zipper &52.7 $\pm$ 3.7 &  49.6 $\pm$ 7.5 & 69 $\pm$ 5.4 & 34.9 $\pm$ 2.8& 58.3 $\pm$ 2.8   & 56.8 $\pm$ 4.0& \textbf{67.8 $\pm$ 6.4} & \textbf{71.4 $\pm$ 9.7} \\
% \midrule
% Avg &69.4 & 63.3& 56.2 & 42.1 & 54.9 & 44.0 & \textbf{74.5}& \textbf{74.5} \\
% \bottomrule \\
% \end{tabular}}

% \caption{ Average AUC  (with standard deviation) for \textbf{One shot} defect detection experiments on MVTec dataset. We denote by "Ours score DD" our model with score calculated using the method of dedect detection. Similarly, we denote by "Ours score AD" our model with score calculated using the method of anomaly detection. Lastly, "OURS score DD DifferNet transforms" is the defect detection score with the same transformations as DifferNet.  %For each dataset, there is one experiment per class, where its training images are used as the images of the normal class. We pick a single image at random from these training images, and train against it. 
% The reported score is the average over $10$ different random images trained on. The same set of images are used for the baseline methods. }
% \label{tab:one_shot_defect}
% \end{table*}

%\begin{table*}
%\centering
%\scalebox{0.8}{%
%\begin{tabular}{cccccccc:cc}
%\toprule 
%\multicolumn{8}{c:} {MVTec } \\
%\midrule
%Class  & DifferNet & DROCC & Patch-SVDD & Deep-SVDD & GEOM & GOAD & \thead{\textbf{OURS} \\ (score DD)} & \thead{\textbf{OURS} \\ (score AD)} & \thead{\textbf{OURS} \\ (score DD \\ DifferNet transforms)} \\
%   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\

%\midrule
%Bottle & \textbf{98.2 $\pm$ 0.4} & 67.2 $\pm$ 6.6 & 60.9 $\pm$ 12.3 & 16.6 $\pm$ 5.3& 79.0 $\pm$ 3.5 & 51.6 $\pm$ 14.0 & 76.3 $\pm$ 6.9 & 62.4 $\pm$ 8.3 & 76.5 $\pm$ 9.0 \\
%Cable & \textbf{76.6 $\pm$ 5.9} & 68.1 $\pm$ 4.3& 58.8 $\pm$ 4.5 & 39.0 $\pm$ 3.5 & 64.2 $\pm$ 1.3 & 47.9 $\pm$ 2.4& 72.3 $\pm$ 3.7 & 64.6 $\pm$ 3.7 & 67.8 $\pm$ 3.6\\
%Capsule &57.7 $\pm$ 4.6& 50.2 $\pm$ 6.4& 57.9 $\pm$ 12.1& 44.8 $\pm$ 4.4& 55.4 $\pm$ 2.6 &51.2 $\pm$ 3.7 &56.0 $\pm$ 8.4 & 46.6 $\pm$ 3.3 & \textbf{59.7 $\pm$ 6.2} \\
%Carpet &61.5 $\pm$3.0 &71.9 $\pm$ 10.6&45.5 $\pm$ 18.8 & 41.2$\pm$ 18.2 & 55.0 $\pm$ 10.1 &48.1 $\pm$ 1.9 & \textbf{72.7 $\pm$ 6.7} & 59.9 $\pm$ 12.9 & \textbf{81.6 $\pm$ 9.2} \\
%Grid &59.2 $\pm$ 5.1 & 50.0 $\pm$ 4.6&37.2 $\pm$ 12.2 & 79.7 $\pm$ 8.6& 40.1 $\pm$ 13.1 & 9.4 $\pm$ 6.8&73.2 $\pm$ 9.8 & 55.3 $\pm$ 4.7 & \textbf{83.3 $\pm$ 7.1} \\
%Hazelnut & \textbf{90.7 $\pm$ 2.7} & 66.4 $\pm$ 7.6 & 46.7 $\pm$ 16.1& 29.1 $\pm$ 4.3& 47.8 $\pm$ 3.6 & 47.6 $\pm$ 3.2 & 82.4 $\pm$ 8.7 &74.2 $\pm$ 7.9 & 69.3 $\pm$ 10.0 \\
%Leather & 83.4 $\pm$ 1.9& 79.1 $\pm$ 6.5& 61.9 $\pm$ 15.6& 48.0 $\pm$ 3.2&  33.2 $\pm$ 0.5 & 58.1 $\pm$ 6.8& \textbf{98.2 $\pm$ 0.9} & 85.0 $\pm$ 5.8 & 96.7 $\pm$ 1.8 \\
%Metalnut & 44.4 $\pm$ 8.0& 51.9 $\pm$ 3.6 & 50.4 $\pm$ 13.1 &42.6 $\pm$ 14.7 & 52.3 $\pm$ 4.2 &7.2 $\pm$ 6.5 & \textbf{66.0 $\pm$ 11.0} & \textbf{84.6 $\pm$ 2.4} & 65.8 $\pm$ 9.9 \\
%Pill & 71.7 $\pm$ 4.4  & \textbf{72.5 $\pm$ 4.0} & 57.6 $\pm$ 8.1& 33.5 $\pm$ 4.0& 67.0 $\pm$ 2.3 & 62.5 $\pm$ 8.1& 56.5 $\pm$ 9.6 & 53.3 $\pm$ 10.1& 66.1 $\pm$ 6.9 \\
%Screw & 61.8 $\pm$ 7.7 & 57.7 $\pm$ 9.0 & 53.7 $\pm$ 18.2& 70.1 $\pm$ 10.8& 34.7 $\pm$ 11.1 & 6.3 $\pm$10.0& \textbf{93.5 $\pm$ 6.2} & 55.0 $\pm$ 6.9 &  89.1 $\pm$ 8.9\\
%Tile & \textbf{87.3 $\pm$ 2.6} & 65.6 $\pm$ 2.0 & 57.3 $\pm$ 4.7 &40.7 $\pm$ 2.8 & 61.0 $\pm$ 2.8 & 6.0 $\pm$ 5.4 & 80.2 $\pm$ 8.2 &60.1 $\pm$ 6.5 &  83.0 $\pm$ 8.9 \\
%Toothbrush &52.1 $\pm$ 2.3 & 68.9 $\pm$ 4.5& 63.7 $\pm$ 6.1 & 35.5 $\pm$ 1.5& 65.7 $\pm$ 6.5 & 54.4$\pm$5.4 &67.3 $\pm$ 4.7 & \textbf{69.3 $\pm$ 3.2} & 57.5 $\pm$ 5.9 \\
%Transistor & 47.0 $\pm$ 6.5& 59.9 $\pm$ 3.3& 66.7 $\pm$ 14.5 &32.8 $\pm$ 4.3 & 58.1 $\pm$ 1.5 & 61.7 $\pm$ 4.4& 66.1 $\pm$ 7.7& \textbf{76.6 $\pm$ 3.6}  & 67.8 $\pm$ 5.8 \\
%Wood & \textbf{96.0 $\pm$ 2.2} & 70.6 $\pm$ 14.4 & 55.7 $\pm$ 18.4 & 44.0 $\pm$ 16.4& 52.3 $\pm$ 1.1 & 41.8 $\pm$ 6.5& 89.0 $\pm$ 4.2 & 45.7 $\pm$ 5.9 & 81.7 $\pm$ 9.9 \\
%Zipper &52.7 $\pm$ 3.7 &  49.6 $\pm$ 7.5 & 69 $\pm$ 5.4 & 34.9 $\pm$ 2.8& 58.3 $\pm$ 2.8   & 56.8 $\pm$ 4.0& \textbf{67.8 $\pm$ 6.4} & 61.2 $\pm$ 6.0 & \textbf{71.4 $\pm$ 9.7} \\
%\midrule
%Avg &69.4 & 63.3& 56.2 & 42.1 & 54.9 & 44.0 & \textbf{74.5} & 63.6 & \textbf{74.5} \\
%\bottomrule \\
%\end{tabular}}

%\caption{ Average AUC  (with standard deviation) for \textbf{One shot} defect detection experiments on MVTec dataset. We denote by "Ours score DD" our model with score calculated using the method of dedect detection. Similarly, we denote by "Ours score AD" our model with score calculated using the method of anomaly detection. Lastly, "OURS score DD DifferNet transforms" is the defect detection score with the same transformations as DifferNet.  %For each dataset, there is one experiment per class, where its training images are used as the images of the normal class. We pick a single image at random from these training images, and train against it. 
%The reported score is the average over $10$ different random images trained on. The same set of images are used for the baseline methods. }
%\label{tab:one_shot_defect}
%\end{table*}


% \noindent  \textbf{Few shot defect detection}
% \sagie{TODO:DESCRIBE THE RESULTS} 

% \begin{table*}
% \centering
% \scalebox{0.8}{%
% \begin{tabular}{cccccccc:c}
% \toprule 
% \multicolumn{8}{c:} {MVTec } \\
% \midrule
% Class  & DifferNet & DROCC & Patch-SVDD & Deep-SVDD & GEOM & GOAD & \thead{\textbf{OURS} \\ (score DD)}  & \thead{\textbf{OURS} \\ (score DD \\ DifferNet transforms)} \\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\

% \midrule
% Bottle & 98.4 $\pm$ 0.2 & 68.1 $\pm$ 2.6 & 61.1 $\pm$ 12.4 & 15.7 $\pm$ 2.8 & 80.0 $\pm$ 1.2 & 51.7 $\pm$ 10.4 &   & 90.8 $\pm$ 3.7 \\
% Cable & 81.3 $\pm$ 2.0 & 68.7 $\pm$ 2.7 & 49 $\pm$ 3.9 & 32.8 $\pm$ 4.9 & 61.1 $\pm$ 3.1 & 46.3 $\pm$ 4.4 & & 76.1 $\pm$ 4.0 \\
% Capsule & 59.0 $\pm$ 2.2 & 53.2 $\pm$ 5.1 &  55.1 $\pm$ 3.4 &  45.3 $\pm$ 4.7 & 60.0 $\pm$ 2.3 &  47.7 $\pm$ 5.9 & & 64.9 $\pm$ 5.6\\
% Carpet & 62.0 $\pm$ 2.2 & 71.6 $\pm$ 10.9 & 46.5 $\pm$ 4.1 &  47.7 $\pm$ 10.5 & 42.2 $\pm$ 6.7 &  44.2 $\pm$ 6.9 & & 65.2 $\pm$ 6.4 \\
% Grid & 56.7 $\pm$ 3.9 & 37.3 $\pm$9.7 & 41.7 $\pm$ 22.1 & 76.0 $\pm$ 11.1 & 36.8 $\pm$ 7.2 & 21.3 $\pm$ 16.4  &  & 82.4 $\pm$ 9.7 \\
% Hazelnut & 93.8 $\pm$ 1.0 & 70.0 $\pm$ 10.9 & 58.6 $\pm$ 17.4 & 27.7 $\pm$ 4.6 & 31.7 $\pm$ 8.2 & 52.5 $\pm$ 3.5  &  & 84.5 $\pm$ 8.8 \\
% Leather & 83.7 $\pm$ 0.8&  70.4 $\pm$ 7.1 & 61.6 $\pm$ 15.4 & 43.0 $\pm$ 2.0 & 33.3 $\pm$ 0.2 & 53.2 $\pm$ 10.3  &   & 98.2 $\pm$ 0.9 \\
% Metalnut &47.2 $\pm$ 3.2 & 59.7 $\pm$ 6.2 & 48.8 $\pm$ 9.1 &  52.9 $\pm$ 6.6 & 36.8 $\pm$ 4.3 & 59.4 $\pm$ 5.6 &  & 76.4 $\pm$ 6.5 \\
% Pill & 79.4 $\pm$ 4.4&  74.4 $\pm$ 3.5 & 57.5 $\pm$ 10.6 & 34.4 $\pm$ 3.5 & 59.1 $\pm$ 3.1 & 61.5 $\pm$ 11.0 & & 63.6 $\pm$ 4.1 \\
% Screw &73.7 $\pm$ 5.1 & 58.3 $\pm$ 2.3&  43.4 $\pm$ 15.1 &  69.5 $\pm$ 3.8 & 18.5 $\pm$ 5.1 & 9.3 $\pm$ 13.6 &  &  74.8 $\pm$ 1.32\\
% Tile & 91.1 $\pm$ 1.4&65.7 $\pm$ 3.1 & 49.5 $\pm$ 3.0 &  32.4 $\pm$ 3.2 & 56.9 $\pm$ 11.1 & 58.6 $\pm$ 3.9 &  & 81.0 $\pm$ 4.4 \\
% Toothbrush &57.3 $\pm$ 3.6 & 67.6 $\pm$ 3.6 & 68.3 $\pm$ 11.8 & 34.9 $\pm$ 6.7 & 72.2 $\pm$ 2.1 & 45.3 $\pm$ 4.5 &  & 64.2 $\pm$ 7.3 \\
% Transistor &55.7 $\pm$ 3.9 & 67.2 $\pm$ 4.1 & 55.3 $\pm$ 9.9 & 30.4 $\pm$ 2.6 & 59.4 $\pm$ 2.9 &  62.8 $\pm$4.0 &  & 76.2 $\pm$ 3.9 \\
% Wood & 96.4 $\pm$ 1.9& 77.7 $\pm$ 11.9 & 69.4 $\pm$ 14.6 & 11.0 $\pm$ 7.3 & 66.0 $\pm$ 9.8 & 37.4 $\pm$ 9.8 &  &  96.2 $\pm$ 1.8 \\
% Zipper & 46.1 $\pm$ 3.7 & 45.2 $\pm$ 6.1 & 63.9$\pm$6.5 & 34.4 $\pm$ 4.6 & 59.2 $\pm$ 6.2 &  54.1 $\pm$ 8. & &  73.3 $\pm$ 10.7 \\
% \midrule
% Avg & 72.1 & 63.7 & 55.3  & 39.2  & 51.5 &  47.0& & 77.9 \\
% \bottomrule \\
% \end{tabular}}

% \caption{ Average AUC  (with standard deviation) for \textbf{Five shot} defect detection experiments on MVTec dataset. We denote by "Ours score DD" our model with score calculated using the method of dedect detection. Similarly, we denote by "Ours score AD" our model with score calculated using the method of anomaly detection. Lastly, "OURS score DD DifferNet transforms" is the defect detection score with the same transformations as DifferNet.  %For each dataset, there is one experiment per class, where its training images are used as the images of the normal class. We pick a single image at random from these training images, and train against it. 
% The reported score is the average over $10$ different random images trained on. The same set of images are used for the baseline methods. }
% \label{tab:five_shot_defect}
% \end{table*}





%\begin{table*}
%\centering
%\scalebox{0.8}{%
%\begin{tabular}{cccccccc:cc}
%\toprule 
%\multicolumn{8}{c:} {MVTec } \\
%\midrule
%Class  & DifferNet & DROCC & Patch-SVDD & Deep-SVDD & GEOM & GOAD & \thead{\textbf{OURS} \\ (score DD)} & \thead{\textbf{OURS} \\ (score AD)} & \thead{\textbf{OURS} \\ (score DD \\ DifferNet transforms)} \\
%   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\

%\midrule
%Bottle & 98.4 $\pm$ 0.2 & 68.1 $\pm$ 2.6 & 61.1 $\pm$ 12.4 & 15.7 $\pm$ 2.8 & 80.0 $\pm$ 1.2 & 51.7 $\pm$ 10.4 &  &51.0 $\pm$ 6.3 & 90.8 $\pm$ 3.7 \\
%Cable & 81.3 $\pm$ 2.0 & 68.7 $\pm$ 2.7 & 49 $\pm$ 3.9 & 32.8 $\pm$ 4.9 & 61.1 $\pm$ 3.1 & 46.3 $\pm$ 4.4 &  & 69.2 $\pm$ 2.5 & 76.1 $\pm$ 4.0 \\
%Capsule & 59.0 $\pm$ 2.2 & 53.2 $\pm$ 5.1 &  55.1 $\pm$ 3.4 &  45.3 $\pm$ 4.7 & 60.0 $\pm$ 2.3 &  47.7 $\pm$ 5.9 & & 44.1 $\pm$ 1.7& 64.9 $\pm$ 5.6\\
%Carpet & 62.0 $\pm$ 2.2 & 71.6 $\pm$ 10.9 & 46.5 $\pm$ 4.1 &  47.7 $\pm$ 10.5 & 42.2 $\pm$ 6.7 &  44.2 $\pm$ 6.9 & & 53.9 $\pm$ 9.6 & 65.2 $\pm$ 6.4 \\
%Grid & 56.7 $\pm$ 3.9 & 37.3 $\pm$9.7 & 41.7 $\pm$ 22.1 & 76.0 $\pm$ 11.1 & 36.8 $\pm$ 7.2 & 21.3 $\pm$ 16.4  & &56.3 $\pm$ 4.9  & 82.4 $\pm$ 9.7 \\
%Hazelnut & 93.8 $\pm$ 1.0 & 70.0 $\pm$ 10.9 & 58.6 $\pm$ 17.4 & 27.7 $\pm$ 4.6 & 31.7 $\pm$ 8.2 & 52.5 $\pm$ 3.5  & & 65.8 $\pm$ 7.1 & 84.5 $\pm$ 8.8 \\
%Leather & 83.7 $\pm$ 0.8&  70.4 $\pm$ 7.1 & 61.6 $\pm$ 15.4 & 43.0 $\pm$ 2.0 & 33.3 $\pm$ 0.2 & 53.2 $\pm$ 10.3  & &92.0 $\pm$ 2.8  & 98.2 $\pm$ 0.9 \\
%Metalnut &47.2 $\pm$ 3.2 & 59.7 $\pm$ 6.2 & 48.8 $\pm$ 9.1 &  52.9 $\pm$ 6.6 & 36.8 $\pm$ 4.3 & 59.4 $\pm$ 5.6 & & 89.5 $\pm$ 3.5 & 76.4 $\pm$ 6.5 \\
%Pill & 79.4 $\pm$ 4.4&  74.4 $\pm$ 3.5 & 57.5 $\pm$ 10.6 & 34.4 $\pm$ 3.5 & 59.1 $\pm$ 3.1 & 61.5 $\pm$ 11.0 & & 47.2 $\pm$ 7.3 & 63.6 $\pm$ 4.1 \\
%Screw &73.7 $\pm$ 5.1 & 58.3 $\pm$ 2.3&  43.4 $\pm$ 15.1 &  69.5 $\pm$ 3.8 & 18.5 $\pm$ 5.1 & 9.3 $\pm$ 13.6 & & 50.9 $\pm$ 8.8 &  74.8 $\pm$ 1.32\\
%Tile & 91.1 $\pm$ 1.4&65.7 $\pm$ 3.1 & 49.5 $\pm$ 3.0 &  32.4 $\pm$ 3.2 & 56.9 $\pm$ 11.1 & 58.6 $\pm$ 3.9 & &74.5 $\pm$ 8.9 & 81.0 $\pm$ 4.4 \\
%Toothbrush &57.3 $\pm$ 3.6 & 67.6 $\pm$ 3.6 & 68.3 $\pm$ 11.8 & 34.9 $\pm$ 6.7 & 72.2 $\pm$ 2.1 & 45.3 $\pm$ 4.5 & & 67.5 $\pm$ 3.6 & 64.2 $\pm$ 7.3 \\
%Transistor &55.7 $\pm$ 3.9 & 67.2 $\pm$ 4.1 & 55.3 $\pm$ 9.9 & 30.4 $\pm$ 2.6 & 59.4 $\pm$ 2.9 &  62.8 $\pm$4.0 & & 83.7 $\pm$ 4.4 & 76.2 $\pm$ 3.9 \\
%Wood & 96.4 $\pm$ 1.9& 77.7 $\pm$ 11.9 & 69.4 $\pm$ 14.6 & 11.0 $\pm$ 7.3 & 66.0 $\pm$ 9.8 & 37.4 $\pm$ 9.8 & & 52.3 $\pm$ 6.1 &  96.2 $\pm$ 1.8 \\
%Zipper & 46.1 $\pm$ 3.7 & 45.2 $\pm$ 6.1 & 63.9$\pm$6.5 & 34.4 $\pm$ 4.6 & 59.2 $\pm$ 6.2 &  54.1 $\pm$ 8. & & 62.7 $\pm$ 5.6 &  73.3 $\pm$ 10.7 \\
%\midrule
%Avg & 72.1 & 63.7 & 55.3  & 39.2  & 51.5 &  47.0& & 64.0 & 77.9 \\
%\bottomrule \\
%\end{tabular}}

%\caption{ Average AUC  (with standard deviation) for \textbf{Five shot} defect detection experiments on MVTec dataset. We denote by "Ours score DD" our model with score calculated using the method of dedect detection. Similarly, we denote by "Ours score AD" our model with score calculated using the method of anomaly detection. Lastly, "OURS score DD DifferNet transforms" is the defect detection score with the same transformations as DifferNet.  %For each dataset, there is one experiment per class, where its training images are used as the images of the normal class. We pick a single image at random from these training images, and train against it. 
%The reported score is the average over $10$ different random images trained on. The same set of images are used for the baseline methods. }
%\label{tab:five_shot_defect}
%\end{table*}


% \begin{table*}
% \centering
% \scalebox{0.8}{%
% \begin{tabular}{cccccccc:c}
% \toprule 
% \multicolumn{8}{c:} {MVTec } \\
% \midrule
% Class  & DifferNet & DROCC & Patch-SVDD & Deep-SVDD & GEOM & GOAD & \thead{\textbf{OURS} \\ (score DD)} & \thead{\textbf{OURS} \\ (score DD \\ DifferNet transforms)} \\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\

% \midrule
% Bottle & \textbf{98.2 $\pm$ 0.4}  & 67.7 $\pm$ 5.1 & 65.3 $\pm$ 9.6 & 17.6 $\pm$ 3.0 & 80.1 $\pm$ 2.5  & 86.9 $\pm$ 4.5 & 81.9 $\pm$ 6.1  & 90.5 $\pm$ 3.1 \\
% Cable & \textbf{82.3 $\pm$ 1.5} & 69.4 $\pm$ 3.0 &  51.1 $\pm$ 7.7 & 32.6 $\pm$ 2.5 & 64.4 $\pm$ 0.8 & 46.0 $\pm$ 9.9 & 73.9 $\pm$ 4.2  & 77.6 $\pm$ 3.9 \\
% Capsule & 58.0 $\pm$ 2.1 & 51.8 $\pm$ 6.3 & 64.4 $\pm$ 11.1 & 44.7 $\pm$ 2.9 & \textbf{65.9 $\pm$ 0.8} & 47.3 $\pm$ 2.0 & 55.8 $\pm$ 7.7 & 59.3 $\pm$ 8.4 \\
% Carpet & 61.8 $\pm$ 1.5 & \textbf{75.1 $\pm$ 16.4} & 49.4 $\pm$ 7.4 &  40.0 $\pm$ 11.6 & 41.4 $\pm$ 7.0 & 50.9 $\pm$ 8.5 & 66.9 $\pm$ 9.6  & 63.9 $\pm$ 6.8 \\
% Grid &58.5 $\pm$ 2.1 &  37.5 $\pm$ 17.1 & 49.8 $\pm$ 11.1 & 67.1 $\pm$ 10.6 & 10.3 $\pm$ 6.7 &  54.0 $\pm$ 7.1 & \textbf{71.0 $\pm$ 8.6} &  \textbf{79.0 $\pm$ 5.9} \\
% Hazelnut & \textbf{93.2 $\pm$ 1.3} & 72.7 $\pm$ 11.9  & 37.9 $\pm$ 12.0 & 30.5 $\pm$ 5.2 & 45.1 $\pm$ 1.6 & 49.6 $\pm$ 2.7 & 72.1 $\pm$ 8.2  & 79.3 $\pm$ 11.3 \\
% Leather & 83.4 $\pm$ 0.9 & 79.1 $\pm$ 13.8 & 49.3 $\pm$ 15.9 & 43.5 $\pm$ 2.8 & 32.7 $\pm$ 0.8 &  61.2 $\pm$ 5.2 & \textbf{99.1 $\pm$ 0.2} & 98.5 $\pm$ 0.5 \\
% Metalnut & 53.4 $\pm$ 7.4 & 59.1 $\pm$ 6.6 & 62.3 $\pm$ 12.5 & 52.4 $\pm$ 3.9 & 49.3 $\pm$ 1.4 & 58.6 $\pm$ 6.7 & 60.4 $\pm$ 11.8  &  74.0 $\pm$ 8.4 \\
% Pill & \textbf{81.8 $\pm$ 3.5} & 77.6 $\pm$ 3.6 & 65.2 $\pm$ 8.4 &  39.1 $\pm$ 3.9 & 56.1 $\pm$ 1.2 & 64.1 $\pm$ 3.0 & 57.4 $\pm$ 10.4 & 66.5 $\pm$ 7.0 \\
% Screw & 78.3 $\pm$ 4.3 & 84.2 $\pm$ 19.8 &  28.8 $\pm$ 21.3 & 65.2 $\pm$ 4.3 & 8.5 $\pm$  6.3 & 66.7 $\pm$ 0.8 & \textbf{93.9 $\pm$ 8.4} & 75.7 $\pm$ 19.0 \\
% Tile & \textbf{91.3 $\pm$ 1.2} & 64.8 $\pm$ 4.2 & 49.0 $\pm$ 3.1 & 26.0 $\pm$ 5.0 & 62.0 $\pm$ 0.3 & 54.3 $\pm$ 3.5 & 87.6 $\pm$ 5.5   & 81.4 $\pm$ 6.9 \\
% Toothbrush & 57.5 $\pm$ 4.0 & 67.9 $\pm$ 3.3 &  67.3 $\pm$ 9.6 & 38.2 $\pm$ 7.6  & 71.5 $\pm$ 0.4 & 51.3 $\pm$ 8.6 & \textbf{78.9 $\pm$ 8.5} &  69.5 $\pm$ 7.7 \\
% Transistor &54.6 $\pm$ 3.7 & 72.5 $\pm$ 3.6 & 60.3 $\pm$ 6.2 & 24.6 $\pm$ 4.5 &58.9 $\pm$ 3.1  & 56.0 $\pm$ 8.4 & \textbf{74.9 $\pm$ 3.7}  & 79.2 $\pm$ 4.7 \\
% Wood & \textbf{96.2 $\pm$ 1.9} &84.0 $\pm$ 8.2  & 47.9 $\pm$ 12.3 &  18.3 $\pm$ 11.6 & 67.7 $\pm$ 5.5 & 37.4 $\pm$ 5.9 & 85.0 $\pm$ 5.9 & 95.8 $\pm$ 1.1 \\
% Zipper & 55.2 $\pm$ 6.1 & 50.0 $\pm$ 6.7 &  66.7 $\pm$ 4.8 & 36.1 $\pm$ 4.5 & 60.9 $\pm$ 2.2 &  53.1 $\pm$ 12.3 & \textbf{72.8 $\pm$ 6.5} &  \textbf{80.4 $\pm$ 5.9} \\
% \midrule
% Avg & 73.6 & 67.6 & 54.3 & 38.4 & 51.6  & 55.8 & \textbf{75.4} & \textbf{78.0} \\
% \bottomrule \\
% \end{tabular}}

% \caption{ Average AUC  (with standard deviation) for \textbf{Ten shot} defect detection experiments on MVTec dataset. We denote by "Ours score DD" our model with score calculated using the method of dedect detection. Similarly, we denote by "Ours score AD" our model with score calculated using the method of anomaly detection. Lastly, "OURS score DD DifferNet transforms" is the defect detection score with the same transformations as DifferNet.  %For each dataset, there is one experiment per class, where its training images are used as the images of the normal class. We pick a single image at random from these training images, and train against it. 
% The reported score is the average over $10$ different random images trained on. The same set of images are used for the baseline methods. }
% \label{tab:ten_shot_defect}
% \end{table*}



%\begin{table*}
%\centering
%\scalebox{0.8}{%
%\begin{tabular}{cccccccc:cc}
%\toprule 
%\multicolumn{8}{c:} {MVTec } \\
%\midrule
%Class  & DifferNet & DROCC & Patch-SVDD & Deep-SVDD & GEOM & GOAD & \thead{\textbf{OURS} \\ (score DD)} & \thead{\textbf{OURS} \\ (score AD)} & \thead{\textbf{OURS} \\ (score DD \\ DifferNet transforms)} \\
%   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\

%\midrule
%Bottle & \textbf{98.2 $\pm$ 0.4}  & 67.7 $\pm$ 5.1 & 65.3 $\pm$ 9.6 & 17.6 $\pm$ 3.0 & 80.1 $\pm$ 2.5  & 86.9 $\pm$ 4.5 & 81.9 $\pm$ 6.1 &57.7 $\pm$ 6.4 & 90.5 $\pm$ 3.1 \\
%Cable & \textbf{82.3 $\pm$ 1.5} & 69.4 $\pm$ 3.0 &  51.1 $\pm$ 7.7 & 32.6 $\pm$ 2.5 & 64.4 $\pm$ 0.8 & 46.0 $\pm$ 9.9 & 73.9 $\pm$ 4.2 &72.1 $\pm$ 2.3 & 77.6 $\pm$ 3.9 \\
%Capsule & 58.0 $\pm$ 2.1 & 51.8 $\pm$ 6.3 & 64.4 $\pm$ 11.1 & 44.7 $\pm$ 2.9 & \textbf{65.9 $\pm$ 0.8} & 47.3 $\pm$ 2.0 & 55.8 $\pm$ 7.7 &  43.5 $\pm$ 2.6 & 59.3 $\pm$ 8.4 \\
%Carpet & 61.8 $\pm$ 1.5 & \textbf{75.1 $\pm$ 16.4} & 49.4 $\pm$ 7.4 &  40.0 $\pm$ 11.6 & 41.4 $\pm$ 7.0 & 50.9 $\pm$ 8.5 & 66.9 $\pm$ 9.6 &54.8 $\pm$ 5.8  & 63.9 $\pm$ 6.8 \\
%Grid &58.5 $\pm$ 2.1 &  37.5 $\pm$ 17.1 & 49.8 $\pm$ 11.1 & 67.1 $\pm$ 10.6 & 10.3 $\pm$ 6.7 &  54.0 $\pm$ 7.1 & \textbf{71.0 $\pm$ 8.6} & 54.0 $\pm$ 4.9 &  \textbf{79.0 $\pm$ 5.9} \\
%Hazelnut & \textbf{93.2 $\pm$ 1.3} & 72.7 $\pm$ 11.9  & 37.9 $\pm$ 12.0 & 30.5 $\pm$ 5.2 & 45.1 $\pm$ 1.6 & 49.6 $\pm$ 2.7 & 72.1 $\pm$ 8.2 &71.8 $\pm$ 7.1  & 79.3 $\pm$ 11.3 \\
%Leather & 83.4 $\pm$ 0.9 & 79.1 $\pm$ 13.8 & 49.3 $\pm$ 15.9 & 43.5 $\pm$ 2.8 & 32.7 $\pm$ 0.8 &  61.2 $\pm$ 5.2 & \textbf{99.1 $\pm$ 0.2} & 93.0 $\pm$ 3.5 & 98.5 $\pm$ 0.5 \\
%Metalnut & 53.4 $\pm$ 7.4 & 59.1 $\pm$ 6.6 & 62.3 $\pm$ 12.5 & 52.4 $\pm$ 3.9 & 49.3 $\pm$ 1.4 & 58.6 $\pm$ 6.7 & 60.4 $\pm$ 11.8 & \textbf{90.3 $\pm$ 2.6}  &  74.0 $\pm$ 8.4 \\
%Pill & \textbf{81.8 $\pm$ 3.5} & 77.6 $\pm$ 3.6 & 65.2 $\pm$ 8.4 &  39.1 $\pm$ 3.9 & 56.1 $\pm$ 1.2 & 64.1 $\pm$ 3.0 & 57.4 $\pm$ 10.4 & 47.2 $\pm$ 7.7 & 66.5 $\pm$ 7.0 \\
%Screw & 78.3 $\pm$ 4.3 & 84.2 $\pm$ 19.8 &  28.8 $\pm$ 21.3 & 65.2 $\pm$ 4.3 & 8.5 $\pm$  6.3 & 66.7 $\pm$ 0.8 & \textbf{93.9 $\pm$ 8.4} & 54.1 $\pm$ 6.4 & 75.7 $\pm$ 19.0 \\
%Tile & \textbf{91.3 $\pm$ 1.2} & 64.8 $\pm$ 4.2 & 49.0 $\pm$ 3.1 & 26.0 $\pm$ 5.0 & 62.0 $\pm$ 0.3 & 54.3 $\pm$ 3.5 & 87.6 $\pm$ 5.5 &70.1 $\pm$ 6.8  & 81.4 $\pm$ 6.9 \\
%Toothbrush & 57.5 $\pm$ 4.0 & 67.9 $\pm$ 3.3 &  67.3 $\pm$ 9.6 & 38.2 $\pm$ 7.6  & 71.5 $\pm$ 0.4 & 51.3 $\pm$ 8.6 & \textbf{78.9 $\pm$ 8.5} & 64.2 $\pm$ 4.9 &  69.5 $\pm$ 7.7 \\
%Transistor &54.6 $\pm$ 3.7 & 72.5 $\pm$ 3.6 & 60.3 $\pm$ 6.2 & 24.6 $\pm$ 4.5 &58.9 $\pm$ 3.1  & 56.0 $\pm$ 8.4 & \textbf{74.9 $\pm$ 3.7}  &\textbf{83.9 $\pm$ 3.4}  & 79.2 $\pm$ 4.7 \\
%Wood & \textbf{96.2 $\pm$ 1.9} &84.0 $\pm$ 8.2  & 47.9 $\pm$ 12.3 &  18.3 $\pm$ 11.6 & 67.7 $\pm$ 5.5 & 37.4 $\pm$ 5.9 & 85.0 $\pm$ 5.9 & 53.9 $\pm$ 3.4 & 95.8 $\pm$ 1.1 \\
%Zipper & 55.2 $\pm$ 6.1 & 50.0 $\pm$ 6.7 &  66.7 $\pm$ 4.8 & 36.1 $\pm$ 4.5 & 60.9 $\pm$ 2.2 &  53.1 $\pm$ 12.3 & \textbf{72.8 $\pm$ 6.5} & 70.0 $\pm$ 7.1 &  \textbf{80.4 $\pm$ 5.9} \\
%\midrule
%Avg & 73.6 & 67.6 & 54.3 & 38.4 & 51.6  & 55.8 & \textbf{75.4} & 65.4 & \textbf{78.0} \\
%\bottomrule \\
%\end{tabular}}

%\caption{ Average AUC  (with standard deviation) for \textbf{Ten shot} defect detection experiments on MVTec dataset. We denote by "Ours score DD" our model with score calculated using the method of dedect detection. Similarly, we denote by "Ours score AD" our model with score calculated using the method of anomaly detection. Lastly, "OURS score DD DifferNet transforms" is the defect detection score with the same transformations as DifferNet.  %For each dataset, there is one experiment per class, where its training images are used as the images of the normal class. We pick a single image at random from these training images, and train against it. 
%The reported score is the average over $10$ different random images trained on. The same set of images are used for the baseline methods. }
%\label{tab:ten_shot_defect}
%\end{table*}



% \subsection{Visualizing our model}

% \begin{figure}
% \centering
% \begin{tabular}{c:c}
% \includegraphics[width=0.5\linewidth]{figures/good.jpg} &
% \includegraphics[width=0.5\linewidth]{figures/bad.jpg} \\
% (a) & (b) 
% % \includegraphics[width=0.95\linewidth]{figures/real_7_mnist.png} & \\
% \end{tabular}
% \begin{tabular}{c:c}
% % \includegraphics[width=0.95\linewidth]{figures/real_7_mnist.png} & \\
% \end{tabular}
% \begin{tabular}{c}
% \includegraphics[width=1\linewidth]{figures/real_7_mnist.png} \\
% (c)
% \end{tabular}
% \caption{Visualization of generated samples in the one shot setting for two different models, (a) and (b), trained on different images of the 7 digit class of MNIST. For both (a) and (b), the train image is shown on the right. Randomly generated samples are shown for each scale, starting from the coarsest scale $0$ and moving up to the finest scale $N=8$.  (c) Random test samples from the MNIST 7 digit class. As can be seen, the model of (a) generates samples (at the final scale 8) which more closely resemble the samples in (c), thus achieving a higher AUC of $80$. On the right, the model less closely resembles the samples in (c) and so it achieves a lower AUC of $55$. { \color{red} HIGHLIGHT CORRECT IN (c)} } 
% \label{fig:visualization}
% \end{figure}






% We consider the effect of training on different images from the normal class. This effect can be best viewed in the one shot setting.
% \shelly{Consider the classes "Defense", "Louvre" and "Pantheon" and three models trained on different training images from this class. In Fig.~\ref{fig:visualization_2} we visualize images that are correctly classified (with the highest "normal" score) in (a)-(b) and incorrectly classified (lowest score) images in (c)-(d).  TODO rephrase: As can be seen from the first row, our model is able to detect distant objects and dark objects,even though the model was trained on centered and illumentaed object. In addition, we can see that is incorrect on objects that are very similar to "defense", and might not differentiate between "Defense" and "Triomphe". Additionally to the dark objects, in the second row we show that our model can handle different orientations of the object that were not shown to the model in training and with hidden objects (the Louver is hided by the human). Last, in the third row we observe one more characteristic of our model in addition to different orientations of the object, darkness and far objects, it can recognize "patches" of the training images and thus correctly classify cropped variants of the object.   }

%Consider the class of digit 7 on MNIST, and two models trained on different training images from this class. We visualize the randomly generated images of both models, for each scale, in Fig.~\ref{fig:visualization}. In particular, a model trained with an image on the left hand side (Fig.~\ref{fig:visualization} (a)), generates random images which more closely resemble the distribution of images in the class of digit 7, as visualized in Fig.~\ref{fig:visualization} (c). This results in getting a high AUC value of 80$\%$. On the right hand side (Fig.~\ref{fig:visualization} (a)), we can see random generated samples which exhibit significantly less variability and less resemble the distribution of images in the class of digit 7. Specifically, the AUC value in this case is  55$\%$. 
%This might be explained by the fact that the training image on the left hand side captures distinctive information about the class, such as, its thickness or edges. On the right hand side, the training image is similar to a $1$ and so many of the generated samples share discriminate features for both the $1$ class and $7$ class. We hypothesize that, the more the training image reflects discriminative details from the class (such color, thickness, corners, change of gradients, contours), the better is our model's performance. 
% The images 
% Furthermore,  we can observe that the thickness of the object affects the quality and credibility of the generated images. 
% This shows that as the training images reflect more the unique details of the class, so our model's performance improved.

%{\color{red}THE UGLIEST SAMPLE EVER}To further support this hypothesis, we consider, in Fig.~\ref{fig:visualization_2}, for the ``sandals'' class of FashionMNIST, the correctly classified test samples of the highest score (least anomalous) and  the incorrectly classified test samples of the lowest score (most anomalous). 
%As can be seen, our model correctly classifies images of a similar patch distribution. In particular, in this case, the model was trained on a thin sandal. Thus, it gives a high score for other thin sandals that resemble the trained image and low score to thick sandals.

%  \noindent\textbf{Defect detection}\quad
% % \paragraph{Defect detection}
% Fig.~\ref{fig:visualization_defect} illustrates the localization of the defects for one shot defect detection, for both our method and that of DifferNet. Three random test samples from MVTec are shown. To visualize these defects, let $D^{n}_x(x_{test})$ be the output of $D^{n}_x$ on a test image $x_{test}$ (original resolution). As $D^{n}_x$ is fully convolutional and dimension preserving, it produces $M+1$ maps of the same spatial dimension as $x_{test}$. Assuming $T_1$ is the identity transformation, we consider map $1$, $D^{n}_x(x_{test})_1$, indicating how real each of the (overlapping) patches of $x_{test}$ are ($T_1(x_{test}) = x_{test})$. The final map is given by the sum of maps $D^{n}_x(x_{test})_1$ (normalized between 0 and 255).
% For DifferNet, we use the visualization procedure provided in their work.
% As can be seen, our method accurately captures the defect regions whereas DifferNet only captures smaller regions of the defect area. 




% \shelly{To ensure $ \{T_1(\overline{x}^n), \dots, T_M(\overline{x}^n)\}$
% belong to $\{p_1^n, \dots, p_M^n\}$, we use Markovian
% %belong to $\{p_1^n_x, \dots, p_M^n_x\}$, we use Markovian
% discriminator $D^n_x$~\cite{CycleGAN2017, disc2}. 
% $D^n_x$ is fully convolutional and uses the same architecture as $G^n_x$ except that the number of output channels in the last convolutional layer is $\mathcal{M} + 1$ (in order to discriminate between patch distributions of different transformed images).}



% \shelly{
% % For this, we define that $ j \in \{1, \dots, M\}$ is the label of  $T_j(\overline{x}^n)$ and $M+1$ is the label of "fake" class. For each transformed image, the discriminator $D^n_x$  outputs a map, which assigns each (overlapping) patch of the input, a vector of size $\mathcal{M} + 1 $ that indicates if the patch belongs to the ``fake'' class or otherwise, for which transformation the patch belongs to. 
% Specifically, for each $T_i$, $D^n_x(T_i(x^n)$ produces $M+1$ maps of size $H \times H$ the number of patches in the map produced by the discriminator. The output shape {\color{red}of XXXX} is $(\mathcal{M} \times (\mathcal{M}+1) \times H \times H)$.  During the adversarial training process,  $G^n_x$ attempts to fool $D^n_x$ into classifying $\{T_1(\overline{x}^n),\dots,T_M(\overline{x}^n)\}$'s patches to the corresponding label of the transformation $\{1, 2, \dots, M\}$, while $D^n_x$ attempts to classify 
% $\{T_1(\overline{x}^n),\dots,T_M(\overline{x}^n)\}$'s 
% patches as fake and $\{T_1({x}^n),\dots,T_M({x}^n)\}$'s 
% to the corresponding label of the transformation 
% $\{1, 2, \dots, M\}$.} 



% \st{To ensure $T_p(\overline{x}^n)$ belongs to $p^n_x$, we employ an adversarial patch-GAN loss using a Markovian discriminator $D^n_x$~\cite{CycleGAN2017, disc2}. $D^n_x$ is fully convolutional and uses the same architecture as $G^n_x$ to produce a map of the same dimension of $T_p(\overline{x}^n)$.} 
% % \shelly{the shape of D's output is not the same as G's output. The shpape of D is (NUM\_TRANSFORM, NUM\_TRANSFORM+1 , NUMBER\_OF\_PATCHES, NUMBER\_OF\_PATCHES) while the output of G is (1,3, SIZE\_AT\_SCALE , SIZE\_AT\_SCALE)}

% \st{
% The map produced by $D^n_x$ assigns each (overlapping) patch of the input, a value that indicates if the patch is real or fake. During the adversarial training process,  $G^n_x$ attempts to fool $D^n_x$ into classifying $T_p(\overline{x}^n)$'s patches as real, while $D^n_x$ attempts to classify $T_p(\overline{x}^n)$'s patches as fake and $T_p(x^n)$'s patches as real.

% The WGAN-GP loss~\cite{wgan-gp} is used for $G^n_x$ and $D^n_x$. Let $\mathbb{M}$ be the mean operator, which is applied to the output of the discriminator $D^n_x$. The loss is computed with respect to the expectation $\mathbb{E}_{T_p}$ over the randomness of $T_p$ (described above):}

% \shelly{The Cross entropy loss is used for $G^n_x$ and $D^n_x$. Let $\mathbb{F}$ be the Flattening operator, which is applied to the output of the discriminator $D^n_x$, and produces a vector of size $(M \cdot H \cdot H, M+1)$. Let $y$ be the target with shape $(M \cdot H \cdot H)$ with values in range $\{1,\dots, M\}$. Denote by [$\vv{M+1}$] the vector of the same shape as $y$ filled with the value $M+1$ indicating the fake class.}
% \begin{align}
% & \mathcal{L}_{adv}(D^n_x, G^n_x) =  CrossEntropy(\mathbb{F}(D^n_x(T_p(x^n))), y) \\ & -  CrossEntropy(\mathbb{F}(D^n_x(T_p(\overline{x}^n))), [\vv{M+1}])
% \end{align}
% \st{where the last term is the gradient penalty of WGAN-GP~\cite{wgan-gp} and is applied to
% % \begin{align}
% % GP^n_x (a, b) = - \lambda \mathbb{E} [(||\nabla_{c} D^n_x(c) -1||_2)^2]
% % \end{align}
% $c = \epsilon \cdot T_p(x^n) + (1-\epsilon) \cdot T_p(\overline{x}^n)$ for $\epsilon$ sampled uniformly between $0$ and $1$, and $\lambda$ is an hyperparameter.} 

% The first term in $\mathcal{L}_{adv}(D^n_x)$ causes $D^n_x$ to maximize the score of the images that lie in $p_x^n$ and to further be classified to the correct class of transformations. The second term, leads it to minimize the score of images that are far from $p_x^n$. \sagie{ELABORATE MORE}
% {\color{red} UNCLEAR SENTENCE. IMPORTANT. PLEASE CLARIFY AND GIVE REFERENCE. This score is proportional the WGAN distance the sample's patch distribution to that of $p^n_x$.}

% One can view $D^n_x$ as maximizing the score of samples in $p^n_x$ while minimizing the score of samples that don't reside in $p^n_x$. This score is proportional the WGAN distance the sample's patch distribution to that of $p^n_x$.


%\textcolor{red}{TODO: OTHER INSIGHTS? }
% \begin{table*}
% \centering

% \scalebox{0.9}{%
% \begin{tabular}{ccccccc}
% \toprule
% Class  & PatchSVDD & DROCC  & Deep-SVDD & GEOM & GOAD & \textbf{GDH(Ours)} \\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\
% \toprule\\
% \multicolumn{7}{c} {PARIS } \\
% \midrule
% Defense & 51.5 $\pm$ 3.3 & \textbf{69.3 $\pm$ 4.5} &  62.1 $\pm$ 3.3  & 59.4 $\pm$ 2.7 & 52.8 $\pm$ 5.1 & 67.8 $\pm$ 3.4 \\
% Eiffel  & 51.2 $\pm$ 4.3 & 66.8 $\pm$ 3.5 &  55.4 $\pm$ 2.8 & 44.1 $\pm$ 6.6 & 53.0 $\pm$ 3.0 & \textbf{67.0 $\pm$ 2.7} \\
% Invalides  &45.2 $\pm$ 2.1  & 62.9 $\pm$ 6.4 & 66.6 $\pm$ 4.9 & 59.2 $\pm$ 2.0 & 52.2 $\pm$ 4.5 & \textbf{80.8 $\pm$ 2.5}  \\
% Louvre   & 41.1 $\pm$ 2.0 & 66.6 $\pm$ 3.3 & 60.4 $\pm$ 4.3  &  53.3 $\pm$ 1.8  & 52.3 $\pm$ 2.7  & \textbf{72.5 $\pm$ 2.8} \\
% Moulinrouge  & 59.6 $\pm$ 3.1 & 44.1 $\pm$ 5.4 & 62.4 $\pm$ 5.1 & 49.0 $\pm$ 0.3 & 45.9 $\pm$ 7.3& \textbf{84.5 $\pm$ 2.4} \\
% Museedorsay   & 53.9 $\pm$ 2.7 & 46.8 $\pm$ 9.6 &  88.0 $\pm$ 3.3 & 88.7 $\pm$ 3.2  &  43.0 $\pm$ 15.2 & \textbf{89.6 $\pm$1.8} \\
% Notredame  & 47.7 $\pm$ 2.8 & 48.7 $\pm$ 6.6 &62.6 $\pm$ 3.5  &   58.4 $\pm$ 1.7   & 48.2 $\pm$5.7  & \textbf{79.7 $\pm$ 4.0}\\
% Pantheon &  58.4 $\pm$ 5.2  & 49.2 $\pm$ 6.6 &  74.9 $\pm$ 2.5 &   60.7 $\pm$ 1.8  &  52.3 $\pm$ 2.3 & \textbf{86.1 $\pm$ 2.1} \\
% Pompidou  & 58.7 $\pm$ 3.4 & 45.7 $\pm$ 7.4 &  75.6 $\pm$ 3.4 & 70.0 $\pm$ 2.7   & 54.1 $\pm$5.8   & \textbf{90.3 $\pm$ 3.4} \\
% Sacrecoeur & 46.9 $\pm$ 7.8 & 58.5 $\pm$ 5.1 & 62.5 $\pm$ 4.3  &  48.1 $\pm$ 0.8   &  54.8 $\pm$ 7.2 & \textbf{81.6 $\pm$ 2.7} \\
% Triomphe & 55.5 $\pm$ 2.6 &47.4 $\pm$ 4.4  &  64.2 $\pm$ 9.4 &    52.4 $\pm$ 1.7 & 51.1 $\pm$ 3.8 & \textbf{78.6 $\pm$ 4.8} \\
% \midrule
% Avg   & 51.8 & 55.1 & 66.8  & 58.5 &50.9 & \textbf{79.8} \\
% \midrule \\
% \multicolumn{7}{c} {CIFAR10 } \\
% \midrule
% Plane & 40.8 $\pm$ 13.8 &  69.0 $\pm$ 4.8& 35.8 $\pm$ 3.1 &62.3 $\pm$ 9.0 & 59.5 $\pm$ 3.0 & \textbf{69.2 $\pm$ 2.8} \\
% Car   & 59.5 $\pm$ 4.5 & 39.6 $\pm$ 8.8 &  74.6 $\pm$ 5.3 &65.5 $\pm$ 7.7 & 68.8 $\pm$10.1& \textbf{77.0 $\pm$ 1.8} \\
% Bird  & 45.7 $\pm$ 6.0 &  \textbf{60.9 $\pm$ 3.4} & 48.4 $\pm$ 5.2  &52.4 $\pm$ 4.8 & 49.4 $\pm$ 3.4 & 58.4 $\pm$ 2.3 \\
% Cat   & 55.6 $\pm$ 3.2 & 56.5 $\pm$ 4.9 & 54.4 $\pm$ 10.7  &54.0 $\pm$ 5.2 & 49.0 $\pm$ 7.0& \textbf{58.7 $\pm$ 4.3} \\
% Deer  & 44.5 $\pm$ 5.3 & 57.9 $\pm$ 5.4 &  51.4 $\pm$ 5.8 & 63.6 $\pm$ 7.6& 48.8 $\pm$ 5.5 & \textbf{66.4 $\pm$ 4.3} \\
% Dog   & 54.4 $\pm$ 3.0 & 59.4 $\pm$ 6.1 & \textbf{70.4 $\pm$ 6.1}  &  55.5 $\pm$ 3.4 &60.9 $\pm$ 11.5 & 61.8 $\pm$ 3.2 \\
% Frog  &  53.7 $\pm$ 5.6& 50.2 $\pm$ 7.7 & 56.0 $\pm$ 5.7 & 58.5 $\pm$ 6.9 &51.5 $\pm$ 2.7 & \textbf{72.6 $\pm$ 4.4} \\
% Horse &   55.4 $\pm$ 3.2 & 43.6 $\pm$ 4.3 & \textbf{69.7 $\pm$ 5.9}  &  64.2 $\pm$3.1 &62.0 $\pm$ 4.9 & 68.6 $\pm$ 2.8 \\
% Ship  &  48.3 $\pm$ 10.3 & 67.5 $\pm$ 6.7 &  73.4 $\pm$ 4.4 & 75.5 $\pm$7.9  & 74.2 $\pm$ 3.6 & \textbf{80.2 $\pm$ 3.2} \\
% Truck & 62.6 $\pm$ 2.2 & 35.9 $\pm$ 5.5 &  70.3 $\pm$ 4.7 &  67.5 $\pm$ 4.0 & \textbf{74.2 $\pm$ 1.7} & 62.1 $\pm$ 4.5\\
% \midrule
% Avg   & 52.1 & 54.1  &  60.4 & 59.5  & 59.9  & \textbf{67.5}   \\
% \midrule \\
% \multicolumn{7}{c} {MNIST } \\
% \midrule
% 0 & 76.6 $\pm$ 2.5 &   70.7 $\pm$ 9.0 &  86.8 $\pm$ 3.2  &  71.3 $\pm$ 6.3  &  \textbf{87.4 $\pm$ 8.0}  & 79.5 $\pm$ 3.8 \\
% 1   & 31.5 $\pm$ 9.9 & 80.6 $\pm$ 7.5 &  89.6 $\pm$ 5.3 & \textbf{96.2 $\pm$ 0.5}   &  89.2 $\pm$ 6.8  & 85.5 $\pm$ 6.7 \\
% 2  & 73.5 $\pm$ 5.2 & 56.4 $\pm$ 10.2 &  73.4 $\pm$ 5.2 &  78.0 $\pm$ 2.6  &  71.3 $\pm$ 7.3  & \textbf{81.6 $\pm$ 4.2} \\
% 3   &  71.0 $\pm$ 5.5& 63.4 $\pm$ 5.3 & 77.2 $\pm$ 10.7  &   85.5 $\pm$ 0.7  & 80.9 $\pm$ 4.6    & \textbf{96.6 $\pm$ 1.0} \\
% 4  &45.0 $\pm$ 5.8  & 69.6 $\pm$ 3.5 & 76.8 $\pm$ 5.8  & 66.4 $\pm$ 5.6   &  70.3 $\pm$ 5.2   & \textbf{84.7 $\pm$ 1.3}  \\
% 5   & 62.6 $\pm$ 3.0 &69.1 $\pm$ 7.2  &  65.6 $\pm$ 6.1 & 79.0 $\pm$ 8.5  & 70.4 $\pm$ 12.8    &  \textbf{89.3 $\pm$ 2.4} \\
% 6  & 55.5 $\pm$ 4.3 & 73.9 $\pm$ 7.5 & 80.0 $\pm$ 5.7 &   76.1 $\pm$ 4.6  &  72.6 $\pm$ 3.9   & \textbf{92.4 $\pm$ 0.9} \\
% 7 &   35.2 $\pm$ 8.3 & 80.4 $\pm$ 7.2 & 81.0 $\pm$ 5.9  &  80.3 $\pm$ 3.8  &   67.1 $\pm$ 5.7  & \textbf{82.0 $\pm$ 3.7} \\
% 8  &  64.9 $\pm$ 6.5& 64.4 $\pm$ 4.6 & \textbf{82.2 $\pm$ 4.4}  &  70.7 $\pm$ 4.0  &73.4 $\pm$ 5.1    & 79.4 $\pm$ 3.4\\
% 9 &  42.2 $\pm$ 6.4& 76.7 $\pm$ 6.3 & 79.2 $\pm$ 4.7  &  65.7 $\pm$ 1.9  &  72.5 $\pm$ 3.9   & \textbf{87.5 $\pm$ 3.2} \\
% \midrule
% Avg   & 55.8 & 70.5 &  79.1 & 76.9  & 75.5& \textbf{85.9} \\
% \midrule \\
% \multicolumn{7}{c} {FashionMNIST } \\
% \midrule
% T-shirt &  52.8 $\pm$ 6.0 &  85.2 $\pm$ 3.1  & 89.6 $\pm$ 2.4  &  \textbf{92.4 $\pm$ 2.7} &  79.8 $\pm$ 2.7 &85.2 $\pm$ 1.7  \\
% Trouser   & 42.2 $\pm$ 10.7 & 94.2 $\pm$ 2.2 &  84.8 $\pm$ 7.1 & 74.7 $\pm$ 2.7  & 97.8 $\pm$ 0.5  & \textbf{98.4 $\pm$ 0.5} \\
% Pullover  &  64.7 $\pm$ 7.0& 80.5 $\pm$ 3.3 & 72.3 $\pm$ 7.1  & 84.3 $\pm$ 3.6  & \textbf{86.4 $\pm$2.2}  & 85.8 $\pm$ 3.5 \\
% Dress   &  41.7 $\pm$ 7.6& 86.3 $\pm$ 4.4  & 77.8 $\pm$ 4.9  &  87.8 $\pm$ 1.0  & 85.1 $\pm$ 2.0   & \textbf{89.1 $\pm$ 2.4} \\
% Coat  &  62.8 $\pm$ 6.1  & 81.5 $\pm$ 3.9  &  76.8 $\pm$ 7.0   &  78.4 $\pm$ 2.0  &  83.8 $\pm$ 1.9  & \textbf{88.4 $\pm$ 1.5} \\
% Sandals   & 60.1 $\pm$ 8.5&  78.1 $\pm$ 15.0  &  63.8 $\pm$ 8.0  & 83.7 $\pm$ 2.0  &  65.9 $\pm$ 7.6  & \textbf{88.6 $\pm$ 2.1}\\
% Shirt &   54.8 $\pm$ 6.6 &  72.0 $\pm$ 3.5  &  \textbf{81.5 $\pm$ 8.0}  &   73.8 $\pm$ 3.7  & 68.0 $\pm$ 3.1   &78.2 $\pm$ 1.7 \\
% Sneaker &  53.0 $\pm$ 10.7  & 93.2 $\pm$ 1.6 & 81.6 $\pm$ 7.4  &  94.6 $\pm$ 1.9  &  94.4 $\pm$ 1.0   & \textbf{99.1 $\pm$ 0.3} \\
% Bag &  53.4 $\pm$ 5.3  &   67.6 $\pm$ 8.7 & 80.1 $\pm$ 3.1    &   \textbf{96.6 $\pm$ 1.4} &   77.5 $\pm$ 6.0 &92.9 $\pm$ 4.1 \\
% Ankle-Boot & 56.4 $\pm$ 9.1 &  90.0 $\pm$ 6.9 & 82.1 $\pm$ 5.4   & 83.7 $\pm$ 4.7  &  \textbf{96.6 $\pm$ 1.5}  &96.5 $\pm$ 1.0 \\
% \midrule
% Avg   &  54.2  &   82.9 &  79.0   &  85.0   &  83.5 &  \textbf{90.2} \\
% \bottomrule \\
% \end{tabular}}
% \caption{\textbf{Five shot} anomaly detection experiments on MNIST, FashionMNIST and CIFAR10 datasets. As in Tab.~\ref{tab:one_shot} $10$ images are chosen at random from the "normal" class. }
% \label{tab:five_shot}
% \end{table*}



% \begin{table*}
% \centering
% \scalebox{0.9}{%
% \begin{tabular}{ccccccc}
% \toprule
% Class  & PatchSVDD & DROCC  & Deep-SVDD & GEOM & GOAD & \textbf{GDH(Ours)}\\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\
% \toprule\\
% \multicolumn{7}{c} {PARIS } \\
% \midrule
% Defense & 54.2 $\pm$ 4.1 & \textbf{72.0 $\pm$ 4.5} &  62.7 $\pm$ 2.3&  57.2 $\pm$ 1.6  &   49.5 $\pm$ 3.3 &67.9 $\pm$ 3.2 \\
% Eiffel  & 48.1 $\pm$ 4.8 & \textbf{73.6 $\pm$ 3.3}  & 59.4 $\pm$ 1.9  & 47.2 $\pm$ 5.6  & 50.0 $\pm$ 0.0   & 71.2 $\pm$ 3.7 \\
% Invalides  & 42.7 $\pm$ 2.8  & 68.0 $\pm$ 4.8 & 67.4 $\pm$ 2.0  & 63.4 $\pm$ 1.0  &  49.9 $\pm$ 0.0  & \textbf{84.9 $\pm$ 1.2}  \\
% Louvre   & 39.4 $\pm$ 1.9 & 73.5 $\pm$ 4.3 &   60.6 $\pm$ 3.3 & 53.4 $\pm$ 1.8   &  49.2 $\pm$ 1.6  & \textbf{74.9 $\pm$ 2.5} \\
% Moulinrouge  & 59.4 $\pm$ 4.3 & 46.6 $\pm$ 2.5 & 63.6 $\pm$ 3.4  &  51.7 $\pm$ 0.8  &  48.8 $\pm$ 2.2  & \textbf{87.0 $\pm$ 3.1} \\
% Museedorsay   & 58.4 $\pm$ 4.0 & 52.3 $\pm$ 3.2 &  89.4 $\pm$ 2.0 & 86.0 $\pm$ 5.1  &    55.5 $\pm$ 6.9 & \textbf{90.7 $\pm$ 2.2} \\
% Notredame  & 52.0 $\pm$ 3.2 & 52.5 $\pm$ 4.6 & 65.8 $\pm$ 2.9  & 55.3 $\pm$ 1.0 &  49.9 $\pm$ 3.1  & \textbf{83.0 $\pm$ 2.9} \\
% Pantheon &  54.5 $\pm$ 4.9  & 57.2 $\pm$ 6.4 & 75.7 $\pm$ 1.6  & 62.3 $\pm$ 0.8 &   50.3 $\pm$ 0.7  &  \textbf{89.9 $\pm$ 2.1} \\
% Pompidou  & 59.9 $\pm$5.6 & 50.3 $\pm$ 4.6 &  77.6 $\pm$ 6.0 & 69.2 $\pm$ 0.8 &   50.2 $\pm$ 2.7  & \textbf{95.4 $\pm$ 1.3} \\
% Sacrecoeur & 48.1 $\pm$ 2.4 & 66.6 $\pm$ 4.9 &66.1 $\pm$ 3.4   & 47.1 $\pm$ 4.1 &   51.2 $\pm$ 3.1  & \textbf{84.5 $\pm$ 1.9} \\
% Triomphe & 59.5 $\pm$ 4.0 & 51.7 $\pm$ 3.9 &  63.3 $\pm$ 10.3 & 53.4 $\pm$ 0.6 &   49.0 $\pm$ 1.1  & \textbf{79.8 $\pm$ 3.4} \\
% \midrule
% Avg   & 52.4  & 60.4 & 68.3   & 58.8      &50.3 & \textbf{82.6} \\
% \midrule \\
% \multicolumn{7}{c} {CIFAR10 } \\
% \midrule
% Plane & 40.8 $\pm$ 9.4 & \textbf{71.9 $\pm$ 2.2} & 39.6 $\pm$ 6.3 & 66.7 $\pm$ 8.8 & 61.5$\pm$2.4 & 69.1 $\pm$ 1.6 \\
% Car   & 59.9 $\pm$ 3.4 & 42.8 $\pm$ 8.2 & 64.0 $\pm$ 9.9  &   74.3 $\pm$ 2.7 & 68.7$\pm$6.1   & \textbf{80.7 $\pm$ 2.9} \\
% Bird  & 44.8 $\pm$ 3.9& \textbf{62.4 $\pm$ 4.4} & 42.4 $\pm$ 11.1  &   54.4 $\pm$ 6.7 &  51.3$\pm$3.2  & 58.5 $\pm$ 2.5 \\
% Cat   & 53.8 $\pm$ 3.7 &61.7 $\pm$ 4.3  &  54.3 $\pm$ 7.3 & 52.5 $\pm$ 5.7  &  50.4$\pm$4.8  & \textbf{63.2 $\pm$ 2.8} \\
% Deer  & 50.1 $\pm$ 4.9 & 62.0 $\pm$ 3.2 & 50.0 $\pm$ 8.7  &  54.1 $\pm$ 5.8 &   52.1 $\pm$ 7.1 & \textbf{64.2 $\pm$ 2.2} \\
% Dog   & 53.3 $\pm$ 4.3 & 61.3 $\pm$ 3.9 & \textbf{81.6 $\pm$ 3.9}   &  60.5 $\pm$ 5.1 &  57.1$\pm$5.7   &65.4 $\pm$ 5.6 \\
% Frog  & 50.4 $\pm$ 4.7 &  48.2 $\pm$ 4.6& 58.0 $\pm$ 11.9 & 60.3 $\pm$ 6.8   &  55.3$\pm$2.3   & \textbf{71.9 $\pm$ 3.3} \\
% Horse & 53.9 $\pm$ 2.9 & 51.6 $\pm$ 3.1 & \textbf{76.8 $\pm$ 5.4}  & 62.9 $\pm$ 4.5   & 61.7$\pm$3.2    &  73.7 $\pm$ 2.8\\
% Ship  &  46.0 $\pm$ 8.5 & 72.6 $\pm$ 3.4 &  71.6 $\pm$ 3.9 &  67.8 $\pm$ 8.7  &  71.3$\pm$2.3   & \textbf{82.9 $\pm$ 0.8} \\
% Truck & 52.6 $\pm$ 4.2 & 39.3 $\pm$ 3.5 &  73.4 $\pm$ 4.2 &  70.3 $\pm$ 4.0  &   \textbf{75.2$\pm$2.5} & 72.6 $\pm$ 2.9\\
% \midrule
% Avg   & 50.5 & 57.4 & 61.1 &  62.4 & 60.5  & \textbf{70.2} \\
% \midrule \\
% \multicolumn{7}{c} {MNIST } \\
% \midrule
% 0 &  75.0 $\pm$ 4.7 & 80.3 $\pm$ 8.0 & \textbf{91.6 $\pm$ 1.1} & 75.0 $\pm$ 1.0   &  72.6 $\pm$ 6.8 &  80.1 $\pm$ 4.6\\
% 1   & 59.3 $\pm$ 13.1 & 78.0 $\pm$ 12.5 & 89.0 $\pm$ 5.8  &  \textbf{96.2 $\pm$ 0.4}  & 90.9 $\pm$ 3.2   &88.8 $\pm$ 3.1  \\
% 2  & 58.6 $\pm$ 5.7 & 58.8 $\pm$ 13.7 & 73.0 $\pm$ 8.8  & 80.1 $\pm$ 2.4   & 68 $\pm$ 5.6  & \textbf{85.2 $\pm$ 4.3} \\
% 3   & 62.0 $\pm$ 6.1 & 66.9 $\pm$ 7.6 & 82.4 $\pm$ 3.2  & 91.0 $\pm$ 0.5   &73.2 $\pm$ 9.3 &  \textbf{96.3 $\pm$ 0.9}\\
% 4  & 53.7 $\pm$ 7.8 & 71.2 $\pm$ 9.8 & 85.6 $\pm$ 0.9  & 79.3 $\pm$ 1.1  &69.1 $\pm$ 6.2 & \textbf{89.1 $\pm$ 1.6} \\
% 5   & 59.8 $\pm$ 5.2 & 63.7 $\pm$ 8.2 &  72.4 $\pm$ 4.0 & 87.2 $\pm$ 0.6  & 62.1 $\pm$ 13.4& \textbf{87.4 $\pm$ 3.3} \\
% 6  & 53.9 $\pm$ 4.8 &  74.0 $\pm$ 14.3  & 88.2 $\pm$ 2.5   & 83.6 $\pm$ 2.8    &73.9 $\pm$ 4.6 & \textbf{92.2 $\pm$ 1.6} \\
% 7 &  50.4 $\pm$ 6.5  & 77.1 $\pm$ 10.8 & 80.0 $\pm$ 7.5  &78.4 $\pm$ 0.7   & 63 $\pm$ 6.5& \textbf{84.2 $\pm$ 4.2} \\
% 8  & 61.5 $\pm$ 4.8 & 69.1 $\pm$ 4.8 & \textbf{81.0 $\pm$ 0.9}  & 64.7 $\pm$ 4.0 &77.8 $\pm$ 5.4 &78.2 $\pm$ 2.3 \\
% 9 & 50.6 $\pm$ 7.0 & 82.9 $\pm$ 6.5 &  82.6 $\pm$ 3.2 &  78.7 $\pm$ 4.8 &67.5 $\pm$ 6.2 & \textbf{90.2 $\pm$ 1.4} \\
% \midrule
% Avg   & 58.5 & 72.2 & 82.6  & 81.4 &  71.8   & \textbf{87.2} \\
% \midrule  \\
% \multicolumn{7}{c} {FashionMNIST } \\
% \midrule
% T-shirt & 50.9 $\pm$ 5.5 &   86.8 $\pm$ 3.3 &  83.5 $\pm$ 2.1 & \textbf{97.5 $\pm$ 0.5}  &  79.7 $\pm$ 3.0 & 86.5 $\pm$ 1.1 \\
% Trouser & 52.9 $\pm$ 12.7 & 94.4 $\pm$ 4.0  & 63.6 $\pm$ 4.6   & 80.2 $\pm$ 0.75 & 97.5 $\pm$ 1.7 & \textbf{99.0 $\pm$ 0.2}    \\
% Pullover & 69.2 $\pm$ 5.8  & 81.2 $\pm$ 3.4 &  66.7 $\pm$ 2.8 & \textbf{90.1 $\pm$ 1.6}  & 89.2 $\pm$ 1.0  & 86.5 $\pm$ 1.1 \\
% Dress   &  36.9 $\pm$ 8.5 & 88.1 $\pm$ 3.6  &  63.1 $\pm$ 0.8 &  91 $\pm$ 1.7  &  87.3 $\pm$ 1.5  & \textbf{91.7 $\pm$ 1.3}  \\
% Coat  &   67.9 $\pm$7.6 &  84.7 $\pm$ 3.5 &  63.6 $\pm$ 4.6  & 88.5 $\pm$ 4.3  & 86.9 $\pm$ 0.9  & \textbf{88.9 $\pm$ 1.2} \\
% Sandals & 54.1 $\pm$ 8.6 & 83.0 $\pm$ 12.4  &  64.9 $\pm$ 6.4  & 86.3 $\pm$ 1.0 & 72.5 $\pm$ 13.1  & \textbf{89.1 $\pm$ 1.6} \\
% Shirt &  55.6 $\pm$ 7.8 & 74.8 $\pm$ 3.8   & 75.1 $\pm$ 3.9   &  \textbf{79.5 $\pm$ 2.5}   &  76.3 $\pm$ 2.0  &78.5 $\pm$ 0.8 \\
% Sneaker &  56.8 $\pm$ 7.8  & 93.3 $\pm$ 1.4 & 59.1 $\pm$ 3.9  &  97.8 $\pm$ 0.4  &  96.3 $\pm$ 1.2  & \textbf{99.0 $\pm$ 0.2} \\
% Bag &  56.1 $\pm$ 8.1  &  73.8 $\pm$ 10.2  &    72.4 $\pm$ 4.6 &  \textbf{98.4 $\pm$ 0.3}  & 77.9 $\pm$2.5   &94.5 $\pm$ 0.4 \\
% Ankle-Boot & 60.3 $\pm$ 12.8   & 85.3 $\pm$ 3.7  &   71.2 $\pm$ 1.1 & 89.6 $\pm$ 0.7  &  97.5 $\pm$ 1.0 & \textbf{98.0 $\pm$ 0.6} \\
% \midrule
% Avg   & 56.1   &  84.5  &   68.3  &   89.9  & 86.1  & \textbf{91.2}  \\
% \bottomrule \\
% \end{tabular}}
% \caption{\textbf{Ten shot} anomaly detection experiments on MNIST, FashionMNIST and CIFAR10 datasets. As in Tab.~\ref{tab:one_shot} $10$ images are chosen at random from the "normal" class. }
% \label{tab:ten_shot}

% \end{table*}

%  \renewcommand\theadfont{}
% \begin{table}
% \centering
% \setlength{\tabcolsep}{3pt} 
% \scalebox{0.75}{%
% \begin{tabular}{ccccccc}
% \toprule
% Class  & PatchSVDD & DROCC  & DeepSVDD & GEOM & GOAD & Ours \\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\
% \toprule\\
% \multicolumn{7}{c} {CIFAR-10 } \\
% \midrule
% Plane &3$6.7\pm6.7$  & $76.2 \pm 2.6 $ & $57.3 \pm 2.6$ & $67.8 \pm 2.9$ & $55.6 \pm 6.4$  &  \\
% Car   & $65.5\pm3.6$  &  $44.7 \pm 3.0$ & $64.1 \pm 1.6$ & $82.4 \pm 1.3$ & $54.3 \pm 7.9$  &  \\
% Bird  & $38.1\pm2.1 $& $66.3 \pm 1.2$ & $46.5 \pm 2.2$ & $60.3 \pm 3.1$ & $52.0 \pm 2.1$  &  \\
% Cat   & $51.3 \pm 3.9$ & $61.4 \pm 4.0$ & $58.5 \pm 2.2$ & $59.6 \pm 5.1$ & $49.8 \pm 0.6$ &  \\
% Deer & $46.3 \pm 4.2$ & 5$8.6 \pm 2.9$ & $53.7 \pm 3.1$ & $57.4 \pm 5.2$ & $50.4 \pm 0.9$  &  \\
% Dog   & $49.4 \pm 3.4$ & $63.3 \pm 5.4$ & $61.7 \pm 2.3$  & $68.6 \pm 2.6$  & $51.8 \pm 3.8$ &  \\
% Frog  & $54.0 \pm 5.6$  & $45.8 \pm 2.6$ & $58.0 \pm 2.7$ & $64.8 \pm 2.8$ & $50.7 \pm 1.0$ &  \\
% Horse & $55.4 \pm 3.1$ & $47.4 \pm 2.6$ & $62.3 \pm 3.2$ & $72.4 \pm 3.1$ & $52.7 \pm 5.4$ &  \\
% Ship  & $44.0 \pm 2.4$ & $74.7 \pm 2.7$ & $75.1 \pm 1.1$ & $81.4 \pm 1.7$ & $59.3 \pm 12.1$ &  \\
% Truck & $60.7 \pm 4.7$ & $37.4 \pm 5.12$ & $71.9 \pm 1.9$ & $81.1 \pm 2.1$ &  $60.4 \pm 11.0$ &  \\
% \midrule
% Avg   &  $50.1$ & $57.6$ & $60.9$  &  $69.6$ & $53.7$ &  \\
% \bottomrule \\
% \end{tabular}}

% \caption{\textbf{50 shot} anomaly detection experiments on CIFAR10 dataset. As in Tab.~\ref{tab:one_shot} but where 5 images are chosen at random from the ``normal'' class. }
% \label{tab:o50_shot_defect}
% \end{table}

%In particular, for the MNIST dataset, in the five shot experiment, the AUC values of our model are the highest for all the classes. 
%On MNIST, our model is still best for the digit $0$ on the five shot setting. Moving to the $10$ shot settings, the best preforming class is digit $6$, indicating that the added variability is significant for this class. 
%On the FashionMNIST dataset, the largest increase in performance between the one-shot on and the few shot setting is for the Ankle-Boot class, for which the added variability is most significant. Similarly, the largest increase in performance occurs for the car class on CIFAR10. 
%We note also that, for Deep-SVDD, the reported average value for CIFAR10, when trained on the full dataset consisting of thousands of images, is $64.8$. This is only slightly higher than the result achieved by our model. 

% {\color{red}See SM for details. HERE NOT SM} 
%\sagie{ADD MORE OR LEAVE TO SUPP. }
% table # compatrs the detection performance on CIFAR-10 for different configurations regarding multi-scaling, the usage of generated samples in training and the usage og transformations in training. Note that we outperform existing methods even without the proposed transformations. 
% \paragraph{Pre-processing} In addition to the transformations mentioned above, we apply histogram equalization technique to the training images in RGB color space. for higher contrast. {\bf IN PROGRESS} }
%\textcolor{red}{TODO SHELLY ELABORATE ON THE TRANSFORMATIONS }
%\st{During  the training of the generative model, in order to further enhance the ability to represent $p^n_{x}$, we augment both real and generated samples, at each scale, with a set of transformations. Unlike other few shot generative models \cite{karras2020training,zhao2020improved}, these transformations are chosen, such that, on one hand, they enrich the sample space captured by the current model, thus enabling it to more faithfully capture $p^n_{x}$, while on the other hand, they do not produce samples outside the class of $x$.} 

%\st{The first set of transformations are \textit{color} changing ones.
%These include the transformation of brightness ($T_1$), contrast ($T_2$), saturation ($T_3$) and hue ($T_4$). The range of possible values for the contrast, saturation and hue is fixed for all input images. In particular, a factor in range $0.6$ to $1.5$ is used for contrast, a factor in range $1.5$ to $4$ is used for saturation and a factor in the range of $-0.05$  to $0.05$ is used for hue. 
%The possible values of brightness, is determined by the brightness of the input image, allowing for bright changes, if the input image is dark, and dark changes if the input image is dark.}

%\st{The transformations are used as part of the adversarial loss. For each scale, for either the real sample $x^n$ or the generated one $\overline{x}^n$, we apply the transformations $T = T_1 \circ \dots \circ T_6$ with a fixed probability $p=0.15$. The choice of transformations $T = T_1 \circ \dots \circ T_6$ and parameter $p$ is the same for all experiments and datasets. We set $T_p(x^n)$ (resp. $T_p(\overline{x}^n)$) to be the result of applying transformations $T$ on $x^n$ (reps. $\overline{x}^n$) with probability $p$. This binary randomness (apply $T$ or not) is on top of the randomness in drawing the transformation $T_1, \dots, T_6$ themselves, which are chosen uniformly from the range of possible values.} 

% Thus, in probability $1-p$ one applies Eq.~\ref{eq:uncon1} and~\ref{eq:uncon2_res} to obtained a reconstructed image, and in probability $p$ one applies the following equations, for a different transformation $T^n$ at each level.

% \begin{align}
% \overline{x}^{0} = G^{0}_x(z^{0}) \label{eq:uncon1}
% \end{align}

% \begin{align}
% \overline{x}^{n} = G^{n}_x(z^n + \uparrow\overline{x}^{n-1})  + \uparrow\overline{x}^{n-1}\,. \label{eq:uncon2_res}
% \end{align}

%\textcolor{red}{TODO: OTHER INSIGHTS?}

% \begin{table*}
% \centering

% \scalebox{0.9}{%
% \begin{tabular}{ccccccc}
% \toprule
% Class  & PatchSVDD & DROCC  & Deep-SVDD & GEOM & GOAD & \textbf{GDH(Ours)} \\
% %   &\cite{schlegl2017unsupervised}  &\cite{bergman2020classification} & \cite{ruff2018deep} &  \\
% \toprule\\
% \multicolumn{7}{c} {PARIS } \\
% \midrule
% Defense & 57.0 $\pm$ 3.5 & 53.2 $\pm$ 8.0 & 50.1 $\pm$5.0 &59.4 $\pm$ 3.1 &  47.8 $\pm$ 5.9 & \textbf{65.6 $\pm$ 9.9} \\ 
% Eiffel  &46.2 $\pm$ 6.2 & 53.3 $\pm$7.9 & 45.8 $\pm$ 6.7  &46.9 $\pm$ 6.0 &  54.6 $\pm$ 3.3 & \textbf{57.8  $\pm$4.5} \\
% Invalides  &46.0 $\pm$ 8.2 & 52.3 $\pm$ 5.1 & 50.3 $\pm$ 6.4   &56.1 $\pm$ 2.9 &  52.9 $\pm$ 3.8  &  \textbf{71.0 $\pm$ 6.4}\\
% Louvre   &  47.3 $\pm$ 5.5 & 57.5 $\pm$ 3.3 & 50.1 $\pm$ 3.0  & 53.7 $\pm$ 4.5 &  52.6 $\pm$ 3.1  & \textbf{61.7  $\pm$ 7.2} \\
% Moulinrouge  & 60.4 $\pm$ 10.2 &43.7 $\pm$ 6.4 & 64.6 $\pm$ 2.1  &9.4 $\pm$ 7.6 &   51.6 $\pm$ 5.9   & \textbf{72.8  $\pm$6.8} \\
% Museedorsay  & 55.7 $\pm$ 8.0 & 42.3 $\pm$ 3.7 & 85.9 $\pm$ 1.9  & \textbf{85.1 $\pm$ 2.7} & 49.3 $\pm$ 16.8  & 73.1 $\pm$ 10.2 \\
% Notredame  & 52.3 $\pm$ 4.8 & 46.9 $\pm$ 4.6 & 58.5 $\pm$ 3.1 &52.2 $\pm$ 5.1  & 49.8 $\pm$ 5.7  & \textbf{66.0  $\pm$ 9.4} \\
% Pantheon & 62.8 $\pm$ 3.7  & 44.2 $\pm$ 6.6 &  54.8 $\pm$ 12.0 &58.5 $\pm$ 7.8 &  49.9 $\pm$ 5.6 & \textbf{73.8  $\pm$ 8.8}  \\
% Pompidou  &56.7 $\pm$ 10.2 & 47.8 $\pm$ 8.9 & 65.5 $\pm$ 3.6  & 65.3 $\pm$ 8.1 &  49 $\pm$ 7.8  & \textbf{68.3  $\pm$9.4}\\
% Sacrecoeur & 55.1 $\pm$ 7.9 & 51.8 $\pm$ 8.4  & 52.1 $\pm$ 4.3  & 48.4 $\pm$ 6.7 &  52 $\pm$ 3.5  & \textbf{61.6  $\pm$ 8.5} \\
% Triomphe & 57.5 $\pm$ 3.8 &  44.2 $\pm$ 5.9 & 59.2 $\pm$ 5.4  & 48.9 $\pm$ 5.6 & 49 $\pm$ 5.7  & \textbf{60.8  $\pm$ 5.5}\\
% \midrule
% Avg   & 54.3 & 48.8 &  57.9  & 56.7 &  50.8 & \textbf{66.6}    \\
% \midrule\\
% \multicolumn{7}{c} {{CIFAR10} } \\
% \midrule 
% Plane &  50.1 $\pm$ 15.8 &    54.9 $\pm$ 9.3&   29.8 $\pm$ 5.5    &  49.5 $\pm$ 11.1  & 59.8 $\pm$ 8.3& \textbf{67.2 $\pm$ 5.8} \\
% Car   & 51.4 $\pm$ 6.3  &   35.2 $\pm$ 7.4  &    \textbf{81.0 $\pm$ 13.5}  & 53.3 $\pm$ 5.7     & 58.2$\pm$ 5.8 & 65.6 $\pm$ 5.9  \\
% Bird  & 46.5 $\pm$ 8.6 &  \textbf{59.5 $\pm$3.7}   &   50.4 $\pm$ 22.4    &54.7 $\pm$ 6.6   & 53.1 $\pm$ 9.1 & 55.9 $\pm$ 5.7 \\
% Cat   &48.9 $\pm$ 6.1  &   52.3 $\pm$ 5.5  &   58.8 $\pm$ 12.7   &53.2 $\pm$ 4.4   &  46.4 $\pm$ 8.2 &  \textbf{58.9 $\pm$ 6.2}\\
% Deer  & 46.5 $\pm$ 10.7 &   65.7 $\pm$ 5.9  &   56.4 $\pm$ 10.6   &\textbf{67.3 $\pm$ 6.4}  &55.9 $\pm$10.7 & 67.2 $\pm$ 4.5 \\
% Dog   & 54.4 $\pm$ 6.3 &    52.7 $\pm$ 8.1 &  22.8 $\pm$ 2.0    &50.9 $\pm$ 2.7 &53.7 $\pm$ 6.0 & \textbf{63.7 $\pm$ 7.7}  \\
% Frog  & 53.4 $\pm$ 17.4 &   53.1 $\pm$ 6.8 &  60.2 $\pm$ 15.9    &60.7 $\pm$ 8.6   & 53.6 $\pm$ 9.9  & \textbf{70.2 $\pm$ 5.1} \\
% Horse &  52.7 $\pm$ 5.1  & 43.5 $\pm$ 6.1&    \textbf{78.6 $\pm$ 13.1}   & 56.0 $\pm$ 4.6    &  54.8 $\pm$ 7.6 &  63.8 $\pm$ 5.2\\
% Ship  &55.6 $\pm$ 13.5 &    57.3 $\pm$ 9.0 &   70.8 $\pm$ 7.9   & 68.1 $\pm$ 10.4    &67.4 $\pm$ 6.4 & \textbf{71.3 $\pm$ 7.2} \\
% Truck & 60.8 $\pm$ 8.1 &     33.6 $\pm$ 5.2&   \textbf{69.8 $\pm$ 6.6}    &57.2 $\pm$ 12.0   & 61.1 $\pm$ 5.5 &65.3 $\pm$ 5.2 \\
% \midrule
% Avg   &  52.0  &50.8  & 57.9      &    57.1 &56.4 & \textbf{64.9}  \\
% \midrule \\
% \multicolumn{7}{c} {{MNIST} } \\
% \midrule 
% 0 & 46.6 $\pm$ 19.4 & 63.4 $\pm$ 14.1 & \textbf{78.6 $\pm$ 12.7} &  73.1 $\pm$ 5.9  & 77.2 $\pm$ 9.1& 75.2 $\pm$ 5.8 \\
% 1   & 82.5 $\pm$ 18.1 & 81.6 $\pm$ 5.6  &  69.8 $\pm$ 7.9 &    \textbf{88.7 $\pm$ 5.0}  & 80.2 $\pm$ 18.3& 79.2 $\pm$ 6.9 \\
% 2  & 56.0 $\pm$ 6.3 & 43.0 $\pm$ 9.2 &67.0 $\pm$ 7.9   & 60.9 $\pm$ 14.4    &72.5 $\pm$ 4.4 &  \textbf{74.3 $\pm$ 3.4} \\
% 3   & 63.1 $\pm$ 1.7 & 54.3 $\pm$ 8.7 & 61.8 $\pm$ 29.4  &  77.0 $\pm$ 3.2   &80.7 $\pm$ 6.9 & \textbf{94.3 $\pm$ 4.8} \\
% 4  & 53.6 $\pm$ 8.4 &59.1 $\pm$ 10.4  &   63.2 $\pm$ 5.1& 66.9 $\pm$ 8.4    & 63.8 $\pm$ 5.9& \textbf{81.6 $\pm$ 7.6} \\
% 5   &60.2 $\pm$ 6.6  & 61.9 $\pm$ 9.5 &   65.2 $\pm$ 4.0& 72.1 $\pm$ 8.3  &54.5 $\pm$ 12.8 & \textbf{80.3 $\pm$ 7.2} \\
% 6  & 59.0 $\pm$ 11.7 & 65.5 $\pm$ 6.7 &  78.2 $\pm$ 4.9&  66.2 $\pm$ 20.2  &70.2 $\pm$ 4.2 & \textbf{85.7 $\pm$ 3.4} \\
% 7 &  49.2 $\pm$ 14.0  & 70.1 $\pm$ 12.0 & 70.2 $\pm$ 3.2  &  69.5 $\pm$ 8.9   & 66.4 $\pm$ 10.3&  \textbf{76.9 $\pm$ 4.0} \\
% 8  & 53.7 $\pm$ 15.6 & 57.5 $\pm$ 7.4 &  \textbf{72.4 $\pm$ 3.7} &   56.2 $\pm$ 2.1  & 71.7 $\pm$ 4.7 & 71.5 $\pm$ 6.2 \\
% 9 & 56.3 $\pm$ 8.9 & 70.3 $\pm$ 7.2 &  61.8 $\pm$ 9.0 &   67.6 $\pm$ 4.3  &59.8 $\pm$ 5.1 & \textbf{73.5 $\pm$ 6.4} \\
% \midrule
% Avg   & 58.0 & 62.7 & 68.8  & 69.8 & 69.7& \textbf{79.3}\\
% \midrule \\
% \multicolumn{7}{c} {{FashionMNIST}} \\
% \midrule 
% T-shirt &  58.5 $\pm$ 5.6&   69.7 $\pm$ 8.1 &  \textbf{83.5 $\pm$ 6.9} &  79.7 $\pm$ 2.9 &  71.8 $\pm$ 14.1  & 77.3 $\pm$ 4.3 \\
% Trouser   & 32.0 $\pm$ 18.6 &  95.2 $\pm$ 1.7 & 63.5 $\pm$ 9.2   &  55.5 $\pm$ 4.3 &  76.0 $\pm$3.7   & \textbf{97.2 $\pm$ 1.4} \\
% Pullover  & 73.7 $\pm$ 8.7 &  68.0 $\pm$ 8.9 &  66.7 $\pm$ 7.3 &  56.9 $\pm$ 12.1   &  69.1 $\pm$5.6   & \textbf{80.3 $\pm$ 4.2} \\
% Dress   & 43.0 $\pm$ 9.8 & 80.9 $\pm$ 6.6   & 63.1 $\pm$ 16.3  &    72.5 $\pm$ 10.5 &   76.9 $\pm$13.1  & \textbf{83.8 $\pm$ 4.0}  \\
% Coat  & 73.3 $\pm$ 4.9 &63.5 $\pm$ 15.1  & 63.6 $\pm$ 12.0  &   52.2 $\pm$ 16.1  &   66.2 $\pm$18.8  &  \textbf{79.0 $\pm$ 9.2} \\
% Sandals  &  39.1 $\pm$ 26.4 & 74.3 $\pm$ 8.4    &64.9 $\pm$ 9.8   &  78.5 $\pm$ 9.7 & 57.9 $\pm$10.1   & \textbf{85.5 $\pm$ 4.5} \\
% Shirt  &  70.2 $\pm$ 2.7 &  64.9 $\pm$ 8.9   &  \textbf{75.1 $\pm$ 6.2}   & 56.1 $\pm$ 5.6   & 72.8 $\pm$3.1    & 69.0 $\pm$ 2.4\\
% Sneaker &  58.1 $\pm$ 25.7 & 90.5 $\pm$ 9.1 &  59.1 $\pm$ 12.0 &  92.6 $\pm$ 2.1  &  69.2 $\pm$1.7   &  \textbf{97.9 $\pm$ 0.7} \\
% Bag  &  70.2 $\pm$ 2.1 &  53.6 $\pm$ 7.4   &  72.4 $\pm$ 3.3  &     \textbf{92.2 $\pm$ 9.1} &  71.7 $\pm$9.9  & 77.2 $\pm$ 15.4\\
% Ankle-Boot & 73.2 $\pm$ 9.2  &  81.9 $\pm$ 14.7   &   71.2 $\pm$ 8.5  &   62.0 $\pm$ 5.8  &   61.6 $\pm$10.6  & \textbf{91.7 $\pm$ 6.1} \\
% \midrule
% Avg   &59.1  & 74.2 &  68.3 &  69.8  & 69.3 &  \textbf{83.9} \\
% \bottomrule \\
% \end{tabular}}

% \caption{ Average AUC  (with standard deviation) for \textbf{One shot} anomaly detection experiments on Paris, CIFAR10, FashionMNIST and MNIST datasets. %For each dataset, there is one experiment per class, where its training images are used as the images of the normal class. We pick a single image at random from these training images, and train against it. 
% The reported score is the average over $10$ different random images trained on. The same set of images are used for the baseline methods. }
% \label{tab:one_shot}

% \end{table*}


% Typically, an anomaly scoring function is devised by approximating the likelihoods of a given data point lying in the underlying distribution, giving a low score to samples having a low likelihood and high otherwise. 
% Approaches differ in the model used to estimate the likelihood of a given sample. 
% Early methods include non-parametric kernel density estimation~\cite{parzen1962estimation}, Gaussian and Gaussian mixture models~\cite{zong2018deep}. These models make strong assumption about the structure of the data, which may not hold in reality. 

